Understanding the One-Pixel Attack: Propagation Maps and Locality Analysis

Deep neural networks were shown to be vulnerable to single pixel modifications. However, the reason behind such phenomena has never been elucidated. Here, we propose Propagation Maps which show the influence of the perturbation in each layer of the network. Propagation Maps reveal that even in extremely deep networks such as Resnet, modification in one pixel easily propagates until the last layer. In fact, this initial local perturbation is also shown to spread becoming a global one and reaching absolute difference values that are close to the maximum value of the original feature maps in a given layer. Moreover, we do a locality analysis in which we demonstrate that nearby pixels of the perturbed one in the one-pixel attack tend to share the same vulnerability, revealing that the main vulnerability lies in neither neurons nor pixels but receptive fields. Hopefully, the analysis conducted in this work together with a new technique called propagation maps shall shed light into the inner workings of other adversarial samples and be the basis of new defense systems to come.

==> unused <==

@inproceedings{mohamed2015variational,
  title={Variational information maximisation for intrinsically motivated reinforcement learning},
  author={Mohamed, Shakir and Rezende, Danilo Jimenez},
  booktitle={Advances in neural information processing systems},
  pages={2125--2133},
  year={2015}
}

@incollection{salge2014empowerment,
  title={Empowerment--an introduction},
  author={Salge, Christoph and Glackin, Cornelius and Polani, Daniel},
  booktitle={Guided Self-Organization: Inception},
  pages={67--114},
  year={2014},
  publisher={Springer}
}

@inproceedings{klyubin2005empowerment,
  title={Empowerment: A universal agent-centric measure of control},
  author={Klyubin, Alexander S and Polani, Daniel and Nehaniv, Chrystopher L},
  booktitle={Evolutionary Computation, 2005. The 2005 IEEE Congress on},
  volume={1},
  pages={128--135},
  year={2005},
  organization={IEEE}
}

@article{vigorito2010intrinsically,
  title={Intrinsically motivated hierarchical skill learning in structured environments},
  author={Vigorito, Christopher M and Barto, Andrew G},
  journal={IEEE Transactions on Autonomous Mental Development},
  volume={2},
  number={2},
  pages={132--143},
  year={2010},
  publisher={IEEE}
}

@inproceedings{chentanez2005intrinsically,
  title={Intrinsically motivated reinforcement learning},
  author={Chentanez, Nuttapong and Barto, Andrew G and Singh, Satinder P},
  booktitle={Advances in neural information processing systems},
  pages={1281--1288},
  year={2005}
}

@article{sutton1999between,
  title={Between MDPs and semi-MDPs: A framework for temporal abstraction in reinforcement learning},
  author={Sutton, Richard S and Precup, Doina and Singh, Satinder},
  journal={Artificial intelligence},
  volume={112},
  number={1-2},
  pages={181--211},
  year={1999},
  publisher={Elsevier}
}

@article{harlow1950learning,
  title={Learning motivated by a manipulation drive.},
  author={Harlow, Harry F and Harlow, Margaret Kuenne and Meyer, Donald R},
  journal={Journal of Experimental Psychology},
  volume={40},
  number={2},
  pages={228},
  year={1950},
  publisher={American Psychological Association}
}

@article{bunzeck2006absolute,
  title={Absolute coding of stimulus novelty in the human substantia nigra/VTA},
  author={Bunzeck, Nico and D{\"u}zel, Emrah},
  journal={Neuron},
  volume={51},
  number={3},
  pages={369--379},
  year={2006},
  publisher={Elsevier}
}

@article{krebs2011novelty,
  title={Novelty increases the mesolimbic functional connectivity of the substantia nigra/ventral tegmental area (SN/VTA) during reward anticipation: Evidence from high-resolution fMRI},
  author={Krebs, RM and Heipertz, Dorothee and Schuetze, Hartmut and Duzel, Emrah},
  journal={Neuroimage},
  volume={58},
  number={2},
  pages={647--655},
  year={2011},
  publisher={Elsevier}
}

@article{weierich2010novelty,
  title={Novelty as a dimension in the affective brain},
  author={Weierich, Mariann R and Wright, Christopher I and Negreira, Alyson and Dickerson, Brad C and Barrett, Lisa Feldman},
  journal={Neuroimage},
  volume={49},
  number={3},
  pages={2871--2878},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{dosovitskiy2014discriminative,
  title={Discriminative unsupervised feature learning with convolutional neural networks},
  author={Dosovitskiy, Alexey and Springenberg, Jost Tobias and Riedmiller, Martin and Brox, Thomas},
  booktitle={Advances in Neural Information Processing Systems},
  pages={766--774},
  year={2014}
}

@misc{deconv,
  title = {Convolution Arithmetic},
  howpublished = {\url{https://github.com/vdumoulin/conv_arithmetic}},
  note = {Accessed: 2017-08-29}
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@misc{VAEtut,
  title = {Variational Autoencoders Explained},
  howpublished = {\url{http://kvfrans.com/variational-autoencoders-explained/}},
  note = {Accessed: 2017-08-29}
}

@article{peng2017deeploco,
  title={DeepLoco: Dynamic locomotion skills using hierarchical deep reinforcement learning},
  author={Peng, Xue Bin and Berseth, Glen and Yin, Kangkang and Van De Panne, Michiel},
  journal={ACM Transactions on Graphics (TOG)},
  volume={36},
  number={4},
  pages={41},
  year={2017},
  publisher={ACM}
}

@inproceedings{zhou2016learning,
  title={Learning deep features for discriminative localization},
  author={Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Oliva, Aude and Torralba, Antonio},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2921--2929},
  year={2016}
}

@article{lin2013network,
  title={Network in network},
  author={Lin, Min and Chen, Qiang and Yan, Shuicheng},
  journal={arXiv preprint arXiv:1312.4400},
  year={2013}
}

@article{takahashi2015tool,
  title={Tool-body assimilation model based on body babbling and neurodynamical system},
  author={Takahashi, Kuniyuki and Ogata, Tetsuya and Tjandra, Hadi and Yamaguchi, Yuki and Sugano, Shigeki},
  journal={Mathematical Problems in Engineering},
  volume={2015},
  year={2015},
  publisher={Hindawi Publishing Corporation}
}

@article{rolf2010goal,
  title={Goal babbling permits direct learning of inverse kinematics},
  author={Rolf, Matthias and Steil, Jochen J and Gienger, Michael},
  journal={IEEE Transactions on Autonomous Mental Development},
  volume={2},
  number={3},
  pages={216--229},
  year={2010},
  publisher={IEEE}
}

@article{bertenthal1996origins,
  title={Origins and early development of perception, action, and representation},
  author={Bertenthal, Bennett I},
  journal={Annual review of psychology},
  volume={47},
  number={1},
  pages={431--459},
  year={1996},
  publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
}

@article{gross1992representation,
  title={Representation of visual stimuli in inferior temporal cortex},
  author={Gross, Charles G and De Schonen, S},
  journal={Philosophical Transactions: Biological Sciences},
  pages={3--10},
  year={1992},
  publisher={JSTOR}
}

@article{van1995functional,
  title={The functional significance of arm movements in neonates},
  author={Van der Meer, ALH and Van der Weel, FR and Lee, David N},
  journal={Science},
  volume={267},
  number={5198},
  pages={693},
  year={1995},
  publisher={The American Association for the Advancement of Science}
}

@article{meltzoff1997explaining,
  title={Explaining facial imitation: A theoretical model},
  author={Meltzoff, Andrew N and Moore, M Keith},
  journal={Early development \& parenting},
  volume={6},
  number={3-4},
  pages={179},
  year={1997},
  publisher={NIH Public Access}
}

@article{ijspeert2008central,
  title={Central pattern generators for locomotion control in animals and robots: a review},
  author={Ijspeert, Auke Jan},
  journal={Neural networks},
  volume={21},
  number={4},
  pages={642--653},
  year={2008},
  publisher={Elsevier}
}

@article{jean2001brain,
  title={Brain stem control of swallowing: neuronal network and cellular mechanisms},
  author={Jean, Andre},
  journal={Physiological reviews},
  volume={81},
  number={2},
  pages={929--969},
  year={2001},
  publisher={Am Physiological Soc}
}

@article{bucher2000central,
  title={Central pattern generators},
  author={Bucher, Dirk and Haspel, Gal and Golowasch, Jorge and Nadim, Farzan},
  journal={eLS},
  year={2000},
  publisher={Wiley Online Library}
}

@article{piaget1971theory,
  title={The theory of stages in cognitive development.},
  author={Piaget, Jean},
  year={1971},
  publisher={McGraw-Hill}
}

@article{zafeiriou2004primitive,
  title={Primitive reflexes and postural reactions in the neurodevelopmental examination},
  author={Zafeiriou, Dimitrios I},
  journal={Pediatric neurology},
  volume={31},
  number={1},
  pages={1--8},
  year={2004},
  publisher={Elsevier}
}

@article{adolph2009handbook,
  title={Handbook of cultural developmental science},
  author={Adolph, KE and Karasik, LB and Tamis-LeMonda, CS},
  year={2009}
}

@article{wiegersma1983motor,
  title={Motor development of deaf children},
  author={Wiegersma, PH and Velde, A Vander},
  journal={Journal of child Psychology and Psychiatry},
  volume={24},
  number={1},
  pages={103--111},
  year={1983},
  publisher={Wiley Online Library}
}


@article{butterfield1986gross,
  title={Gross motor profiles of deaf children},
  author={Butterfield, Stephen A},
  journal={Perceptual and motor skills},
  volume={62},
  number={1},
  pages={68--70},
  year={1986},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}


@article{levtzion2000early,
  title={Early motor development of blind children},
  author={Levtzion-Korach, Osnat and Tennenbaum, Alex and Schnitzer, Robert and Ornoy, Asher},
  journal={Journal of paediatrics and child health},
  volume={36},
  number={3},
  pages={226--229},
  year={2000},
  publisher={Wiley Online Library}
}

@article{schott2003grasp,
  title={The grasp and other primitive reflexes},
  author={Schott, JM and Rossor, MN},
  journal={Journal of Neurology, Neurosurgery \& Psychiatry},
  volume={74},
  number={5},
  pages={558--560},
  year={2003},
  publisher={BMJ Publishing Group Ltd}
}


@inproceedings{saegusa2009active,
  title={Active motor babbling for sensorimotor learning},
  author={Saegusa, Ryo and Metta, Giorgio and Sandini, Giulio and Sakka, Sophie},
  booktitle={Robotics and Biomimetics, 2008. ROBIO 2008. IEEE International Conference on},
  pages={794--799},
  year={2009},
  organization={IEEE}
}


@article{levin1999babbling,
  title={Babbling in infants with cerebral palsy},
  author={Levin, Karen},
  journal={Clinical linguistics \& phonetics},
  volume={13},
  number={4},
  pages={249--267},
  year={1999},
  publisher={Taylor \& Francis}
}

@book{mccomas1996skeletal,
  title={Skeletal muscle: form and function},
  author={McComas, Alan J},
  year={1996},
  publisher={Champaign, IL: Human Kinetics}
}


@article{brooks2003current,
  title={Current topics for teaching skeletal muscle physiology},
  author={Brooks, Susan V},
  journal={Advances in physiology education},
  volume={27},
  number={4},
  pages={171--182},
  year={2003},
  publisher={Am Physiological Soc}
}

@article{welsh1997some,
  title={Some organizing principles for the control of movement based on olivocerebellar physiology},
  author={Welsh, John P and Llin{\'a}s, Rodolfo},
  journal={Progress in brain research},
  volume={114},
  pages={449--461},
  year={1997},
  publisher={Elsevier}
}


@book{haykin2004comprehensive,
 author = {Haykin, Simon},
 title = {Neural Networks: A Comprehensive Foundation},
 year = {1998},
 isbn = {0132733501},
 edition = {2nd},
 publisher = {Prentice Hall PTR},
 address = {Upper Saddle River, NJ, USA},
} 

@article{vigorito2010intrinsically,
  title={Intrinsically motivated hierarchical skill learning in structured environments},
  author={Vigorito, Christopher M and Barto, Andrew G},
  journal={Autonomous Mental Development, IEEE Transactions on},
  volume={2},
  number={2},
  pages={132--143},
  year={2010},
  publisher={IEEE}
}

@article{botvinick2014model,
  title={Model-based hierarchical reinforcement learning and human action control},
  author={Botvinick, Matthew and Weinstein, Ari},
  journal={Philosophical Transactions of the Royal Society of London B: Biological Sciences},
  volume={369},
  number={1655},
  pages={20130480},
  year={2014},
  publisher={The Royal Society}
}

@article{mcgovern2001automatic,
  title={Automatic discovery of subgoals in reinforcement learning using diverse density},
  author={McGovern, Amy and Barto, Andrew G},
  journal={Computer Science Department Faculty Publication Series},
  pages={8},
  year={2001}
}

@article{moradi2012automatic,
  title={Automatic skill acquisition in reinforcement learning using graph centrality measures},
  author={Moradi, Parham and Shiri, Mohammad Ebrahim and Rad, Ali Ajdari and Khadivi, Alireza and Hasler, Martin},
  journal={Intelligent Data Analysis},
  volume={16},
  number={1},
  pages={113--135},
  year={2012},
  publisher={IOS Press}
}




@article{maia2011reinforcement,
  title={From reinforcement learning models to psychiatric and neurological disorders},
  author={Maia, Tiago V and Frank, Michael J},
  journal={Nature neuroscience},
  volume={14},
  number={2},
  pages={154--162},
  year={2011},
  publisher={Nature Publishing Group}
}

@article{watson1913psychology,
  title={Psychology as the behaviorist views it.},
  author={Watson, John B},
  journal={Psychological review},
  volume={20},
  number={2},
  pages={158},
  year={1913},
  publisher={Psychological Review Company}
}

@book{sutton1998introduction,
  title={Introduction to reinforcement learning},
  author={Sutton, Richard S and Barto, Andrew G},
  volume={135},
  year={1998},
  publisher={MIT Press Cambridge}
}

@book{koza1992genetic,
  title={Genetic programming: on the programming of computers by means of natural selection},
  author={Koza, John R},
  volume={1},
  year={1992},
  publisher={MIT press}
}

@incollection{miller2000cartesian,
  title={Cartesian genetic programming},
  author={Miller, Julian F and Thomson, Peter},
  booktitle={Genetic Programming},
  pages={121--132},
  year={2000},
  publisher={Springer}
}

@inproceedings{lessin2014adapting,
  title={Adapting morphology to multiple tasks in evolved virtual creatures},
  author={Lessin, Dan and Fussell, Don and Miikkulainen, Risto},
  booktitle={ALIFE 14: The Fourteenth Conference on the Synthesis and Simulation of Living Systems},
  volume={14},
  pages={247--254}
}
@inproceedings{sutskever2014sequence,
  title={Sequence to sequence learning with neural networks},
  author={Sutskever, Ilya and Vinyals, Oriol and Le, Quoc V},
  booktitle={Advances in neural information processing systems},
  pages={3104--3112},
  year={2014}
}
@article{collobert2011natural,
  title={Natural language processing (almost) from scratch},
  author={Collobert, Ronan and Weston, Jason and Bottou, L{\'e}on and Karlen, Michael and Kavukcuoglu, Koray and Kuksa, Pavel},
  journal={The Journal of Machine Learning Research},
  volume={12},
  pages={2493--2537},
  year={2011},
  publisher={JMLR. org}
}

@article{alipanahi2015predicting,
  title={Predicting the sequence specificities of DNA-and RNA-binding proteins by deep learning},
  author={Alipanahi, Babak and Delong, Andrew and Weirauch, Matthew T and Frey, Brendan J},
  journal={Nature biotechnology},
  year={2015},
  publisher={Nature Publishing Group}
}


@article{zhou2015predicting,
  title={Predicting effects of noncoding variants with deep learning-based sequence model},
  author={Zhou, Jian and Troyanskaya, Olga G},
  journal={Nature methods},
  volume={12},
  number={10},
  pages={931--934},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{gawehn2015deep,
  title={Deep Learning in Drug Discovery},
  author={Gawehn, Erik and Hiss, Jan A and Schneider, Gisbert},
  journal={Molecular Informatics},
  year={2015},
  publisher={Wiley Online Library}
}

@inproceedings{koutnik2013evolving,
  title={Evolving large-scale neural networks for vision-based reinforcement learning},
  author={Koutn{\'\i}k, Jan and Cuccu, Giuseppe and Schmidhuber, J{\"u}rgen and Gomez, Faustino},
  booktitle={Proceedings of the 15th annual conference on Genetic and evolutionary computation},
  pages={1061--1068},
  year={2013},
  organization={ACM}
}

@book{banzhaf1998genetic,
  title={Genetic programming: an introduction},
  author={Banzhaf, Wolfgang and Nordin, Peter and Keller, Robert E and Francone, Frank D},
  volume={270},
  year={1998},
  publisher={Morgan Kaufmann San Francisco}
}


@article{ghahramani2015probabilistic,
  title={Probabilistic machine learning and artificial intelligence},
  author={Ghahramani, Zoubin},
  journal={Nature},
  volume={521},
  number={7553},
  pages={452--459},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{maddison2014move,
  title={Move evaluation in go using deep convolutional neural networks},
  author={Maddison, Chris J and Huang, Aja and Sutskever, Ilya and Silver, David},
  journal={arXiv preprint arXiv:1412.6564},
  year={2014}
}

@misc{TORCS,
author = "Bernhard Wymann, Eric Espi{\'e}, Christophe Guionneau, Christos Dimitrakakis, R{\'e}mi Coulom, Andrew Sumner",
howpublished = "http://www.torcs.org",
title = "{TORCS}, {T}he {O}pen {R}acing {C}ar {S}imulator",
year = "2014",
}

@ARTICLE{bellemare13arcade,
  author = {{Bellemare}, M.~G. and {Naddaf}, Y. and {Veness}, J. and {Bowling}, M.},
  title = {The Arcade Learning Environment: An Evaluation Platform for General Agents},
  journal = {Journal of Artificial Intelligence Research},
  year = 2013,
  month = 06,
  volume = 47,
  pages = {253--279}
}

@article{mersmann2015analyzing,
  title={Analyzing the bbob results by means of benchmarking concepts},
  author={Mersmann, Olaf and Preuss, Mike and Trautmann, Heike and Bischl, Bernd and Weihs, Claus},
  journal={Evolutionary computation},
  volume={23},
  number={1},
  pages={161--185},
  year={2015},
  publisher={MIT Press}
}

@article{weston2014memory,
  title={Memory networks},
  author={Weston, Jason and Chopra, Sumit and Bordes, Antoine},
  journal={arXiv preprint arXiv:1410.3916},
  year={2014}
}

@article{graves2014neural,
  title={Neural turing machines},
  author={Graves, Alex and Wayne, Greg and Danihelka, Ivo},
  journal={arXiv preprint arXiv:1410.5401},
  year={2014}
}

@inproceedings{yamins2013hierarchical,
  title={Hierarchical modular optimization of convolutional networks achieves representations similar to macaque IT and human ventral stream},
  author={Yamins, Daniel L and Hong, Ha and Cadieu, Charles and DiCarlo, James J},
  booktitle={Advances in neural information processing systems},
  pages={3093--3101},
  year={2013}
}

@article{lorenz2011emergence,
  title={The emergence of modularity in biological systems},
  author={Lorenz, Dirk M and Jeng, Alice and Deem, Michael W},
  journal={Physics of life reviews},
  volume={8},
  number={2},
  pages={129--160},
  year={2011},
  publisher={Elsevier}
}

@article{clune2013evolutionary,
  title={The evolutionary origins of modularity},
  author={Clune, Jeff and Mouret, Jean-Baptiste and Lipson, Hod},
  journal={Proceedings of the Royal Society of London B: Biological Sciences},
  volume={280},
  number={1755},
  pages={20122863},
  year={2013},
  publisher={The Royal Society}
}

@article{cully2015robots,
  title={Robots that can adapt like animals},
  author={Cully, Antoine and Clune, Jeff and Tarapore, Danesh and Mouret, Jean-Baptiste},
  journal={Nature},
  volume={521},
  number={7553},
  pages={503--507},
  year={2015},
  publisher={Nature Publishing Group}
}


@inproceedings{huizinga2014evolving,
  title={Evolving neural networks that are both modular and regular: HyperNeat plus the connection cost technique},
  author={Huizinga, Joost and Clune, Jeff and Mouret, Jean-Baptiste},
  booktitle={Proceedings of the 2014 conference on Genetic and evolutionary computation},
  pages={697--704},
  year={2014},
  organization={ACM}
}

@article{stanley2009hypercube,
  title={A hypercube-based encoding for evolving large-scale neural networks},
  author={Stanley, Kenneth O and D'Ambrosio, David B and Gauci, Jason},
  journal={Artificial life},
  volume={15},
  number={2},
  pages={185--212},
  year={2009},
  publisher={MIT Press}
}

@article{mersmann2015analyzing,
  title={Analyzing the bbob results by means of benchmarking concepts},
  author={Mersmann, Olaf and Preuss, Mike and Trautmann, Heike and Bischl, Bernd and Weihs, Claus},
  journal={Evolutionary computation},
  volume={23},
  number={1},
  pages={161--185},
  year={2015},
  publisher={MIT Press}
}

@article{reehuis2011model,
  title={Model-guided Evolution Strategies for Dynamically Balancing Exploration and Exploitation},
  author={Reehuis, Edgar and Kruisselbrink, Johannes and Olhofer, Markus and Graening, Lars and Sendhoff, Bernhard and B{\"a}ck, Thomas},
  journal={Artificial Evolution 2011 (Evolution Artificielle 2011)},
  publisher={Citeseer}
}

@article{lehman2008exploiting,
  title={Exploiting open-endedness to solve problems through the search for novelty},
  author={Lehman, J. and Stanley, K.O.},
  journal={Artificial Life},
  volume={11},
  pages={329},
  year={2008}
}

@inproceedings{cuccu2011novelty,
  title={Novelty-based restarts for evolution strategies},
  author={Cuccu, Giuseppe and Gomez, Faustino and Glasmachers, Tobias},
  booktitle={Evolutionary Computation (CEC), 2011 IEEE Congress on},
  pages={158--163},
  year={2011},
  organization={IEEE}
}

@article{stanley2007compositional,
  title={Compositional pattern producing networks: A novel abstraction of development},
  author={Stanley, Kenneth O},
  journal={Genetic programming and evolvable machines},
  volume={8},
  number={2},
  pages={131--162},
  year={2007},
  publisher={Springer}
}

@article{kohl2012integrated,
  title={An integrated neuroevolutionary approach to reactive control and high-level strategy},
  author={Kohl, Nate and Miikkulainen, Risto},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={16},
  number={4},
  pages={472--488},
  year={2012},
  publisher={IEEE}
}

@inproceedings{kohl2008evolving,
  title={Evolving neural networks for fractured domains},
  author={Kohl, Nate and Miikkulainen, Risto},
  booktitle={Proceedings of the 10th annual conference on Genetic and evolutionary computation},
  pages={1405--1412},
  year={2008},
  organization={ACM}
}

@techreport{ethembabaoglu2008automatic,
  title={Automatic feature selection using FS-NEAT},
  author={Ethembabaoglu, Aksel and Whiteson, Shimon},
  year={2008},
  institution={Technical report IAS-UVA-08-02, Intelligent Autonomous Systems Group, University of Amsterdam}
}

@incollection{clune2007investigating,
  title={Investigating the emergence of phenotypic plasticity in evolving digital organisms},
  author={Clune, Jeff and Ofria, Charles and Pennock, Robert T},
  booktitle={Advances in Artificial Life},
  pages={74--83},
  year={2007},
  publisher={Springer}
}

@article{hornik1989multilayer,
  title={Multilayer feedforward networks are universal approximators},
  author={Hornik, Kurt and Stinchcombe, Maxwell and White, Halbert},
  journal={Neural networks},
  volume={2},
  number={5},
  pages={359--366},
  year={1989},
  publisher={Elsevier}
}

@PhdThesis{gruau1994neural,
  title={Neural Network Synthesis using Cellular Encoding and the Genetic Algorithm.},
  author={Gruau, Frederic and others},
  year={1994},
  school={Ecole Normale Superieure de Lyon}
}


@article{moriarty1997forming,
  title={Forming neural networks through efficient and adaptive coevolution},
  author={Moriarty, David E and Miikkulainen, Risto},
  journal={Evolutionary Computation},
  volume={5},
  number={4},
  pages={373--399},
  year={1997},
  publisher={MIT Press}
}

@article{saravanan1995evolving,
  title={Evolving neural control systems},
  author={Saravanan, Natarajan and Fogel, David B},
  journal={IEEE Intelligent Systems},
  volume={10},
  number={3},
  pages={23--27},
  year={1995},
  publisher={IEEE Computer Society}
}

@inproceedings{wieland1991evolving,
  title={Evolving neural network controllers for unstable systems},
  author={Wieland, Alexis P},
  booktitle={Neural Networks, 1991., IJCNN-91-Seattle International Joint Conference on},
  volume={2},
  pages={667--673},
  year={1991},
  organization={IEEE}
}


@article{whitley1993genetic,
  title={Genetic Reinforcement Learning for Neurocontrol Problems},
  author={Whitley, Darrell and Dominic, Stephen and Das, Rajarshi and Anderson, Charles W},
  journal={Machine Learning},
  volume={13},
  pages={259--284},
  year={1993}
}

@article{siebel2007evolutionary,
  title={Evolutionary reinforcement learning of artificial neural networks},
  author={Siebel, Nils T and Sommer, Gerald},
  journal={International Journal of Hybrid Intelligent Systems},
  volume={4},
  number={3},
  pages={171--183},
  year={2007},
  publisher={IOS Press}
}

@book{anthony2009neural,
  title={Neural network learning: Theoretical foundations},
  author={Anthony, Martin and Bartlett, Peter L},
  year={2009},
  publisher={cambridge university press}
}


@article{nakata2015xcs,
  title={XCS-SL: a rule-based genetic learning system for sequence labeling},
  author={Nakata, Masaya and Kovacs, Tim and Takadama, Keiki},
  journal={Evolutionary Intelligence},
  pages={1--16},
  year={2015},
  publisher={Springer}
}

@article{kohl2012integrated,
  title={An integrated neuroevolutionary approach to reactive control and high-level strategy},
  author={Kohl, Nate and Miikkulainen, Risto},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={16},
  number={4},
  pages={472--488},
  year={2012},
  publisher={IEEE}
}

@inproceedings{gauci2007generating,
  title={Generating large-scale neural networks through discovering geometric regularities},
  author={Gauci, Jason and Stanley, Kenneth},
  booktitle={Proceedings of the 9th annual conference on Genetic and evolutionary computation},
  pages={997--1004},
  year={2007},
  organization={ACM}
}

@book{koza1992genetic,
  title={Genetic programming: on the programming of computers by means of natural selection},
  author={Koza, John R},
  volume={1},
  year={1992},
  publisher={MIT press}
}

@article{orriols2009fuzzy,
  title={Fuzzy-UCS: a Michigan-style learning fuzzy-classifier system for supervised learning},
  author={Orriols-Puig, Albert and Casillas, Jorge and Bernad{\'o}-Mansilla, Ester},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={13},
  number={2},
  pages={260--283},
  year={2009},
  publisher={IEEE}
}

@article{rosenstein2004supervised,
  title={Supervised Actor-Critic Reinforcement Learning},
  author={Rosenstein, Michael T and Barto, Andrew G and Si, Jennie and Barto, Andy and Powell, Warren and Wunsch, Donald},
  journal={Handbook of Learning and Approximate Dynamic Programming},
  pages={359--380},
  year={2004},
  publisher={Wiley Online Library}
}

@incollection{starzyk2010novel,
  title={A Novel Optimization Algorithm Based on Reinforcement Learning},
  author={Starzyk, Janusz A and Liu, Yinyin and Batog, Sebastian},
  booktitle={Computational Intelligence in Optimization},
  pages={27--47},
  year={2010},
  publisher={Springer}
}

@article{berglund2006parameterless,
  title={The parameterless self-organizing map algorithm},
  author={Berglund, Erik and Sitte, Joaquin},
  journal={Neural Networks, IEEE Transactions on},
  volume={17},
  number={2},
  pages={305--316},
  year={2006},
  publisher={IEEE}
}

@inproceedings{miagkikh1999global,
  title={Global search in combinatorial optimization using reinforcement learning algorithms},
  author={Miagkikh, Victor V and Punch III, William F},
  booktitle={Evolutionary Computation, 1999. CEC 99. Proceedings of the 1999 Congress on},
  volume={1},
  year={1999},
  organization={IEEE}
}

@article{grondman2012survey,
  title={A Survey of Actor-Critic Reinforcement Learning: Standard and Natural Policy Gradients},
  author={Grondman, Ivo and Busoniu, Lucian and Lopes, Gabriel AD and Babuska, Robert},
  journal={Systems, Man, and Cybernetics, Part C: Applications and Reviews, IEEE Transactions on},
  volume={42},
  number={6},
  pages={1291--1307},
  year={2012},
  publisher={IEEE}
}

@article{shao2013swarm,
  title={Swarm robots reinforcement learning convergence accuracy-based learning classifier systems with gradient descent (XCS-GD)},
  author={Shao, Jie and Lin, Haixia and Zhang, Kaibian},
  journal={Neural Computing and Applications},
  pages={1--6},
  year={2013},
  publisher={Springer}
}

@article{kober2013reinforcement,
  title={Reinforcement learning in robotics: A survey},
  author={Kober, Jens and Bagnell, J Andrew and Peters, Jan},
  journal={The International Journal of Robotics Research},
  volume={32},
  number={11},
  pages={1238--1274},
  year={2013},
  publisher={SAGE Publications}
}

@article{van2011insights,
  title={Insights in Reinforcement Learning: formal analysis and empirical evaluation of temporal-difference learning algorithms},
  author={van Hasselt, HP},
  journal={SIKS dissertation series},
  volume={2011},
  number={04},
  year={2011},
  publisher={Utrecht University}
}

@article{barto1983neuronlike,
  title={Neuronlike adaptive elements that can solve difficult learning control problems},
  author={Barto, Andrew G and Sutton, Richard S and Anderson, Charles W},
  journal={Systems, Man and Cybernetics, IEEE Transactions on},
  number={5},
  pages={834--846},
  year={1983},
  publisher={IEEE}
}

@article{rougier2011dynamic,
  title={Dynamic self-organising map},
  author={Rougier, Nicolas and Boniface, Yann},
  journal={Neurocomputing},
  volume={74},
  number={11},
  pages={1840--1847},
  year={2011},
  publisher={Elsevier}
}


@article{yao1997new,
  title={A new evolutionary system for evolving artificial neural networks},
  author={Yao, Xin and Liu, Yong},
  journal={Neural Networks, IEEE Transactions on},
  volume={8},
  number={3},
  pages={694--713},
  year={1997},
  publisher={IEEE}
}

@inproceedings{kassahun2005efficient,
  title={Efficient reinforcement learning through evolutionary acquisition of neural topologies},
  author={Kassahun, Yohannes and Sommer, Gerald},
  booktitle={In 13th European Symposium on Artificial Neural Networks (ESANN)},
  year={2005},
  organization={Citeseer}
}

@article{angeline1994evolutionary,
  title={An evolutionary algorithm that constructs recurrent neural networks},
  author={Angeline, Peter J and Saunders, Gregory M and Pollack, Jordan B},
  journal={Neural Networks, IEEE Transactions on},
  volume={5},
  number={1},
  pages={54--65},
  year={1994},
  publisher={IEEE}
}

@Misc{neatcode,
author = {Stanley, K. and Karpov, I. V. and Bahceci, E. and D'Silva, T.},
title = {{NEAT C++}},
howpublished = {\url{http://nn.cs.utexas.edu/keyword?neat-c}},
year = {2001--2011}
}

@article{gers2003learning,
  title={Learning precise timing with LSTM recurrent networks},
  author={GERS, Felix A and SCHRAUDOLPH, Nicol N and SCHMIDHUBER, J{\"u}rgen},
  journal={Journal of machine learning research},
  volume={3},
  number={1},
  pages={115--143},
  year={2003},
  publisher={MIT Press}
}

@article{kohl:nn09,
title={Evolving Neural Networks for Strategic Decision-Making Problems},
author={Nate Kohl and Risto Miikkulainen},
booktitle={Neural Networks, Special issue on Goal-Directed Neural Systems},
url="http://nn.cs.utexas.edu/?kohl:nn09",
year={2009}
}

@inproceedings{kohl2008evolving,
  title={Evolving neural networks for fractured domains},
  author={Kohl, Nate and Miikkulainen, Risto},
  booktitle={Proceedings of the 10th annual conference on Genetic and evolutionary computation},
  pages={1405--1412},
  year={2008},
  organization={ACM}
}

@article{whiteson2006evolutionary,
  title={Evolutionary function approximation for reinforcement learning},
  author={Whiteson, Shimon and Stone, Peter},
  journal={The Journal of Machine Learning Research},
  volume={7},
  pages={877--917},
  year={2006},
  publisher={JMLR. org}
}

@inproceedings{gomez1999solving,
  title={Solving non-Markovian control tasks with neuroevolution},
  author={Gomez, Faustino J and Miikkulainen, Risto},
  booktitle={IJCAI},
  volume={99},
  pages={1356--1361},
  year={1999}
}

@article{stanley2002evolving,
  title={Evolving neural networks through augmenting topologies},
  author={Stanley, Kenneth and Miikkulainen, Risto},
  journal={Evolutionary computation},
  volume={10},
  number={2},
  pages={99--127},
  year={2002},
  publisher={MIT Press}
}

@article{stanley1996efficient,
  title={Efficient reinforcement learning through evolving neural network topologies},
  author={Stanley, Kenneth O and Miikkulainen, Risto},
  journal={Network (Phenotype)},
  volume={1},
  number={2},
  pages={3},
  year={1996}
}

@inproceedings{sutton1996generalization,
  title={Generalization in Reinforcement Learning: Successful Examples Using Sparse Coarse Coding},
  author={Sutton, Richard S},
  booktitle={Advances in Neural Information Processing Systems 8},
  year={1996}
}

@incollection{bonarini1996evolutionary,
  title={Evolutionary learning of fuzzy rules: competition and cooperation},
  author={Bonarini, Andrea},
  booktitle={Fuzzy Modelling},
  pages={265--283},
  year={1996},
  publisher={Springer}
}

@InProceedings{Twardowski1993a,
  author =       "Kirk Twardowski",
  title =        "{Credit Assignment for Pole Balancing with Learning
                 Classifier Systems}",
  pages =        "238--245",
  crossref =     "ICGA93",
  keywords =     "LCS",
  abstract =     "Effective reinforcement learning methods are essential
                 for credit assignment in learning classifier systems in
                 order to guide the structural rule-base modifications
                 performed by genetic algorithms. Currently, a number of
                 algorithms have been proposed to fulfill this
                 fundamental need; the most frequently employed being
                 the bucket-brigade algorithm. In this paper, an
                 experimental evaluation of a number of reinforcement
                 learning algorithms for a variety of parameter settings
                 is presented. A simplified learning classifier system
                 is used in order to minimize system complexity in order
                 to isolate the behavior of the reinforcement learning
                 algorithms. The problem domain tackled is that of the
                 control of an unstable dynamic system. It was
                 discovered that exploitation of current information is
                 highly favored over exploration for new information and
                 that a hybrid bucket brigade-backward averaging
                 algorithm produced the fastest convergence to a
                 solution.",
}


@article{deb2002fast,
  title={A fast and elitist multiobjective genetic algorithm: NSGA-II},
  author={Deb, Kalyanmoy and Pratap, Amrit and Agarwal, Sameer and Meyarivan, TAMT},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={6},
  number={2},
  pages={182--197},
  year={2002},
  publisher={IEEE}
}

@article{lehman2010abandoning,
  title={Abandoning objectives: Evolution through the search for novelty alone},
  author={Lehman, J. and Stanley, K.O.},
  journal={Evolutionary Computation},
  pages={1--34},
  year={2010},
  publisher={MIT Press}
}

@inproceedings{doncieux2009exploring,
  title={Exploring new horizons in evolutionary design of robots},
  author={Doncieux, S. and Mouret, J.B. and Bredeche, N.},
  booktitle={Workshop on Exploring new horizons in Evolutionary Design of Robots at IROS},
  volume={2009},
  pages={5--12},
  year={2009}
}

@inproceedings{doncieux2010behavioral,
  title={Behavioral diversity measures for evolutionary robotics},
  author={Doncieux, S. and Mouret, J.B.},
  booktitle={Evolutionary Computation (CEC), 2010 IEEE Congress on},
  pages={1--8},
  year={2010},
  organization={IEEE}
}

@inproceedings{lehman2010efficiently,
  title={Efficiently evolving programs through the search for novelty},
  author={Lehman, J. and Stanley, K.O.},
  booktitle={Proceedings of the 12th annual conference on Genetic and evolutionary computation},
  pages={837--844},
  year={2010},
  organization={ACM}
}

@inproceedings{mouret2009using,
  title={Using behavioral exploration objectives to solve deceptive problems in neuro-evolution},
  author={Mouret, J.B. and Doncieux, S.},
  booktitle={Proceedings of the 11th Annual conference on Genetic and evolutionary computation},
  pages={627--634},
  year={2009},
  organization={ACM}
}

@article{xiong2007non,
  title={A non-stationary covariance-based Kriging method for metamodelling in engineering design},
  author={Xiong, Ying and Chen, Wei and Apley, Daniel and Ding, Xuru},
  journal={International Journal for Numerical Methods in Engineering},
  volume={71},
  number={6},
  pages={733--756},
  year={2007},
  publisher={Wiley Online Library}
}

@inproceedings{reehuis2011model,
  title={Model-guided Evolution Strategies for Dynamically Balancing Exploration and Exploitation},
  author={Reehuis, Edgar and Kruisselbrink, Johannes and Olhofer, Markus and Graening, Lars and Sendhoff, Bernhard and B{\"a}ck, Thomas},
  booktitle={Artificial Evolution},
  pages={306--317},
  year={2011}
}

@inproceedings{schaul2011curiosity,
  title={Curiosity-driven optimization},
  author={Schaul, Tom and Sun, Yi and Wierstra, Daan and Gomez, Fausino and Schmidhuber, J{\"u}rgen},
  booktitle={Evolutionary Computation (CEC), 2011 IEEE Congress on},
  pages={1343--1349},
  year={2011},
  organization={IEEE}
}

@inproceedings{hester2012intrinsically,
  title={Intrinsically motivated model learning for a developing curious agent},
  author={Hester, Todd and Stone, Peter},
  booktitle={Development and Learning and Epigenetic Robotics (ICDL), 2012 IEEE International Conference on},
  pages={1--6},
  year={2012},
  organization={IEEE}
}

%----------------------- Anomaly Detection --------------------------

@article{chandola2009anomaly,
  title={Anomaly detection: A survey},
  author={Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  journal={ACM computing surveys (CSUR)},
  volume={41},
  number={3},
  pages={15},
  year={2009},
  publisher={ACM}
}

@article{patcha2007overview,
  title={An overview of anomaly detection techniques: Existing solutions and latest technological trends},
  author={Patcha, Animesh and Park, Jung-Min},
  journal={Computer networks},
  volume={51},
  number={12},
  pages={3448--3470},
  year={2007},
  publisher={Elsevier}
}

@article{hodge2004survey,
  title={A survey of outlier detection methodologies},
  author={Hodge, Victoria J and Austin, Jim},
  journal={Artificial intelligence review},
  volume={22},
  number={2},
  pages={85--126},
  year={2004},
  publisher={Springer}
}

@article{bamnett1994outliers,
  title={Outliers in statistical data},
  author={Bamnett, V and Lewis, T},
  year={1994},
  publisher={JSTOR}
}

@book{rousseeuw2005robust,
  title={Robust regression and outlier detection},
  author={Rousseeuw, Peter J and Leroy, Annick M},
  volume={589},
  year={2005},
  publisher={John Wiley \& Sons}
}

@book{jain1988algorithms,
  title={Algorithms for clustering data},
  author={Jain, Anil K and Dubes, Richard C},
  year={1988},
  publisher={Prentice-Hall, Inc.}
}

@article{jain1999data,
  title={Data clustering: a review},
  author={Jain, Anil K and Murty, M Narasimha and Flynn, Patrick J},
  journal={ACM computing surveys (CSUR)},
  volume={31},
  number={3},
  pages={264--323},
  year={1999},
  publisher={Acm}
}

@inproceedings{steven1988smaha,
  title={SMAHA. Haystack: an intrusion detection system},
  author={Steven, E},
  booktitle={Proceedings of the Fourth Aerospace Computer Security Applications Conference},
  volume={44},
  year={1988},
  organization={Washington: IEEE Computer Society Press}
}

@misc{anderson1995next,
  title={Next-generation intrusion detection expert system (NIDES): A summary},
  author={Anderson, Debra and Frivold, Thane and Valdes, Alfonso},
  year={1995},
  publisher={SRI International, Computer Science Laboratory Menio Park, CA}
}

@inproceedings{portnoy2001intrusion,
  title={Intrusion detection with unlabeled data using clustering},
  author={Portnoy, Leonid and Eskin, Eleazar and Stolfo, Sal},
  booktitle={In Proceedings of ACM CSS Workshop on Data Mining Applied to Security (DMSA-2001)},
  year={2001},
  organization={Citeseer}
}

@inproceedings{leung2005unsupervised,
  title={Unsupervised anomaly detection in network intrusion detection using clusters},
  author={Leung, Kingsly and Leckie, Christopher},
  booktitle={Proceedings of the Twenty-eighth Australasian conference on Computer Science-Volume 38},
  pages={333--342},
  year={2005},
  organization={Australian Computer Society, Inc.}
}

@article{simard2005using,
  title={Using machine learning to break visual human interaction proofs (hips)},
  author={Simard, PY},
  journal={Advances in neural information processing systems},
  volume={17},
  pages={265--272},
  year={2005}
}

@inproceedings{forrest1996sense,
  title={A sense of self for unix processes},
  author={Forrest, Stephanie and Hofmeyr, Steven A and Somayaji, Anil and Longstaff, Thomas A},
  booktitle={Security and Privacy, 1996. Proceedings., 1996 IEEE Symposium on},
  pages={120--128},
  year={1996},
  organization={IEEE}
}

@inproceedings{kruegel2003bayesian,
  title={Bayesian event classification for intrusion detection},
  author={Kruegel, Christopher and Mutz, Darren and Robertson, William and Valeur, Fredrik},
  booktitle={Computer Security Applications Conference, 2003. Proceedings. 19th Annual},
  pages={14--23},
  year={2003},
  organization={IEEE}
}

@inproceedings{ye2000probabilistic,
  title={Probabilistic networks with undirected links for anomaly detection},
  author={Ye, Nong and Xu, Mingming and Emran, Syed Masum},
  booktitle={IEEE Systems, Man, and Cybernetics Information Assurance and Security Workshop},
  pages={175--179},
  year={2000}
}

@inproceedings{valdes2000adaptive,
  title={Adaptive, model-based monitoring for cyber attack detection},
  author={Valdes, Alfonso and Skinner, Keith},
  booktitle={International Workshop on Recent Advances in Intrusion Detection},
  pages={80--93},
  year={2000},
  organization={Springer}
}

@inproceedings{warrender1999detecting,
  title={Detecting intrusions using system calls: Alternative data models},
  author={Warrender, Christina and Forrest, Stephanie and Pearlmutter, Barak},
  booktitle={Security and Privacy, 1999. Proceedings of the 1999 IEEE Symposium on},
  pages={133--145},
  year={1999},
  organization={IEEE}
}

@article{yeung2003host,
  title={Host-based intrusion detection using dynamic and static behavioral models},
  author={Yeung, Dit-Yan and Ding, Yuxin},
  journal={Pattern recognition},
  volume={36},
  number={1},
  pages={229--243},
  year={2003},
  publisher={Elsevier}
}

@article{lippmann20001999,
  title={The 1999 DARPA off-line intrusion detection evaluation},
  author={Lippmann, Richard and Haines, Joshua W and Fried, David J and Korba, Jonathan and Das, Kumar},
  journal={Computer networks},
  volume={34},
  number={4},
  pages={579--595},
  year={2000},
  publisher={Elsevier}
}

@article{ye2002multivariate,
  title={Multivariate statistical analysis of audit trails for host-based intrusion detection},
  author={Ye, Nong and Emran, Syed Masum and Chen, Qiang and Vilbert, Sean},
  journal={IEEE Transactions on Computers},
  volume={51},
  number={7},
  pages={810--820},
  year={2002},
  publisher={IEEE}
}

@inproceedings{lee1998data,
  title={Data Mining Approaches for Intrusion Detection.},
  author={Lee, Wenke and Stolfo, Salvatore J and others},
  booktitle={Usenix security},
  year={1998}
}

@inproceedings{dickerson2000fuzzy,
  title={Fuzzy network profiling for intrusion detection},
  author={Dickerson, John E and Dickerson, Julie A},
  booktitle={Fuzzy Information Processing Society, 2000. NAFIPS. 19th International Conference of the North American},
  pages={301--306},
  year={2000},
  organization={IEEE}
}

@inproceedings{bridges2000fuzzy,
  title={Fuzzy data mining and genetic algorithms applied to intrusion detection},
  author={Bridges, Susan M and Vaughn, Rayford B},
  booktitle={Proceedings of 12th Annual Canadian Information Technology Security Symposium},
  pages={109--122},
  year={2000}
}

@article{han2005evolutionary,
  title={Evolutionary neural networks for anomaly detection based on the behavior of a program},
  author={Han, Sang-Jun and Cho, Sung-Bae},
  journal={IEEE Transactions on Systems, Man, and Cybernetics, Part B (Cybernetics)},
  volume={36},
  number={3},
  pages={559--570},
  year={2005},
  publisher={IEEE}
}

@inproceedings{ghosh1999study,
  title={A Study in Using Neural Networks for Anomaly and Misuse Detection.},
  author={Ghosh, Anup K and Schwartzbard, Aaron},
  booktitle={USENIX Security},
  year={1999}
}

@inproceedings{crosbie1995applying,
  title={Applying genetic programming to intrusion detection},
  author={Crosbie, Mark and Spafford, Gene},
  booktitle={Working Notes for the AAAI Symposium on Genetic Programming},
  pages={1--8},
  year={1995},
  organization={Cambridge, MA: MIT Press}
}

@article{zhang2008random,
  title={Random-forests-based network intrusion detection systems},
  author={Zhang, Jiong and Zulkernine, Mohammad and Haque, Anwar},
  journal={IEEE Transactions on Systems, Man, and Cybernetics, Part C (Applications and Reviews)},
  volume={38},
  number={5},
  pages={649--659},
  year={2008},
  publisher={IEEE}
}

@inproceedings{wressnegger2013close,
  title={A close look on n-grams in intrusion detection: anomaly detection vs. classification},
  author={Wressnegger, Christian and Schwenk, Guido and Arp, Daniel and Rieck, Konrad},
  booktitle={Proceedings of the 2013 ACM workshop on Artificial intelligence and security},
  pages={67--76},
  year={2013},
  organization={ACM}
}

@inproceedings{wang2006anagram,
  title={Anagram: A content anomaly detector resistant to mimicry attack},
  author={Wang, Ke and Parekh, Janak J and Stolfo, Salvatore J},
  booktitle={International Workshop on Recent Advances in Intrusion Detection},
  pages={226--248},
  year={2006},
  organization={Springer}
}

@inproceedings{forrest1996sense,
  title={A sense of self for unix processes},
  author={Forrest, Stephanie and Hofmeyr, Steven A and Somayaji, Anil and Longstaff, Thomas A},
  booktitle={Security and Privacy, 1996. Proceedings., 1996 IEEE Symposium on},
  pages={120--128},
  year={1996},
  organization={IEEE}
}

@inproceedings{jacob2012static,
  title={A static, packer-agnostic filter to detect similar malware samples},
  author={Jacob, Gr{\'e}goire and Comparetti, Paolo Milani and Neugschwandtner, Matthias and Kruegel, Christopher and Vigna, Giovanni},
  booktitle={International Conference on Detection of Intrusions and Malware, and Vulnerability Assessment},
  pages={102--122},
  year={2012},
  organization={Springer}
}

@inproceedings{laskov2011static,
  title={Static detection of malicious JavaScript-bearing PDF documents},
  author={Laskov, Pavel and {\v{S}}rndi{\'c}, Nedim},
  booktitle={Proceedings of the 27th Annual Computer Security Applications Conference},
  pages={373--382},
  year={2011},
  organization={ACM}
}

@inproceedings{koch2014towards,
  title={Towards Comparability of Intrusion Detection Systems: New Data Sets},
  author={Koch, Robert and Golling, Mario and Rodosek, Gabi Dreo},
  booktitle={TERENA Networking Conference},
  pages={7},
  year={2014}
}

@article{weller2015survey,
  title={A survey of distance and similarity measures used within network intrusion anomaly detection},
  author={Weller-Fahy, David J and Borghetti, Brett J and Sodemann, Angela A},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={17},
  number={1},
  pages={70--91},
  year={2015},
  publisher={IEEE}
}

@article{lin2015cann,
  title={CANN: An intrusion detection system based on combining cluster centers and nearest neighbors},
  author={Lin, Wei-Chao and Ke, Shih-Wen and Tsai, Chih-Fong},
  journal={Knowledge-based systems},
  volume={78},
  pages={13--21},
  year={2015},
  publisher={Elsevier}
}

@article{kim2014novel,
  title={A novel hybrid intrusion detection method integrating anomaly detection with misuse detection},
  author={Kim, Gisung and Lee, Seungmin and Kim, Sehun},
  journal={Expert Systems with Applications},
  volume={41},
  number={4},
  pages={1690--1700},
  year={2014},
  publisher={Elsevier}
}



%----------------------- My publications --------------------------

@article{vargasspectrum,
  title={Spectrum-Diverse Neuroevolution With Unified Neural Models},
  author={Vargas, Danilo Vasconcellos and Murata, Junichi},
  journal={IEEE Transactions on Neural Networks and Learning Systems}
}


@article{vargas2015general,
  title={General subpopulation framework and taming the conflict inside populations},
  author={Vargas, Danilo Vasconcellos and Murata, Junichi and Takano, Hirotaka and Delbem, Alexandre Cl{\'a}udio Botazzo},
  journal={Evolutionary computation},
  volume={23},
  number={1},
  pages={1--36},
  year={2015},
  publisher={MIT Press}
}

@inproceedings{vargas2013aself,
  title={Self organizing classifiers and niched fitness},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi},
  booktitle={Proceedings of the fifteenth annual conference on Genetic and evolutionary computation conference},
  pages={1109--1116},
  year={2013},
  organization={ACM}
}

@inproceedings{vargas2015novelty,
  title={Novelty-organizing team of classifiers in noisy and dynamic environments},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi},
  booktitle={Evolutionary Computation (CEC), 2015 IEEE Congress on},
  pages={2937--2944},
  year={2015},
  organization={IEEE}
}


@inproceedings{vargas2014novelty,
  title={Novelty-organizing team of classifiers-A team-individual multi-objective approach to reinforcement learning},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi},
  booktitle={SICE Annual Conference (SICE), 2014 Proceedings of the},
  pages={1785--1792},
  year={2014},
  organization={IEEE}
}

@inproceedings{vargas2013continuous,
  title={Continuous adaptive reinforcement learning with the evolution of Self Organizing Classifiers},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi},
  booktitle={Development and Learning and Epigenetic Robotics (ICDL), 2013 IEEE Third Joint International Conference on},
  pages={1--2},
  year={2013},
  organization={IEEE}
}

@article{vargas2013self,
  title={Self organizing classifiers: first steps in structured evolutionary machine learning},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi},
  journal={Evolutionary Intelligence},
  volume={6},
  number={2},
  pages={57--72},
  year={2013},
  publisher={Springer}
}

@inproceedings{vargas2014noc,
  author    = {Danilo Vasconcellos Vargas and
               Hirotaka Takano and
               Junichi Murata},
  title     = {Novelty-organizing classifiers applied to classification and reinforcement
               learning: towards flexible algorithms},
  booktitle = {Genetic and Evolutionary Computation Conference, {GECCO} '14, Vancouver,
               BC, Canada, July 12-16, 2014, Companion Material Proceedings},
  pages     = {81--82},
  year      = {2014}
}

  
%------------------------------------------------------------------



@inproceedings{knox2010combining,
  title={Combining manual feedback with subsequent MDP reward signals for reinforcement learning},
  author={Knox, W Bradley and Stone, Peter},
  booktitle={Proceedings of the 9th International Conference on Autonomous Agents and Multiagent Systems: volume 1-Volume 1},
  pages={5--12},
  year={2010},
  organization={International Foundation for Autonomous Agents and Multiagent Systems}
}


@article{igel2004no,
  title={{A no-free-lunch theorem for non-uniform distributions of target functions}},
  author={Igel, C. and Toussaint, M.},
  journal={Journal of Mathematical Modelling and Algorithms},
  volume={3},
  number={4},
  pages={313--322},
  issn={1570-1166},
  year={2004},
  publisher={Springer}
}

@article{franco2013gassist,
  title={GAssist vs. BioHEL: critical assessment of two paradigms of genetics-based machine learning},
  author={Franco, Mar{\'\i}a A and Krasnogor, Natalio and Bacardit, Jaume},
  journal={Soft Computing},
  pages={1--29},
  year={2013},
  publisher={Springer}
}

@incollection{bacardit2007data,
  title={Data mining in learning classifier systems: comparing XCS with GAssist},
  author={Bacardit, Jaume and Butz, Martin V},
  booktitle={Learning Classifier Systems},
  pages={282--290},
  year={2007},
  publisher={Springer}
}

@misc{uci2013,
author = "K. Bache and M. Lichman",
year = "2013",
title = "{UCI} Machine Learning Repository",
url = "http://archive.ics.uci.edu/ml",
institution = "University of California, Irvine, School of Information and Computer Sciences" 
} 

@article{unold2005context,
  title={Context-free grammar induction with grammar-based classifier system},
  author={Unold, O},
  journal={Archives of Control Science},
  volume={15},
  number={4},
  pages={681},
  year={2005},
  publisher={POLITECHNIKA SLASKA}
}

@article{dam2008neural,
  title={Neural-based learning classifier systems},
  author={Dam, Hai Huong and Abbass, Hussein A and Lokan, Chris and Yao, Xin},
  journal={Knowledge and Data Engineering, IEEE Transactions on},
  volume={20},
  number={1},
  pages={26--39},
  year={2008},
  publisher={IEEE}
}

@article{wilson2002classifiers,
  title={Classifiers that approximate functions},
  author={Wilson, Stewart W},
  journal={Natural Computing},
  volume={1},
  number={2-3},
  pages={211--234},
  year={2002},
  publisher={Springer}
}

@article{floreano2008neuroevolution,
  title={Neuroevolution: from architectures to learning},
  author={Floreano, Dario and D{\"u}rr, Peter and Mattiussi, Claudio},
  journal={Evolutionary Intelligence},
  volume={1},
  number={1},
  pages={47--62},
  year={2008},
  publisher={Springer}
}

@article{holmes2002learning,
  title={Learning classifier systems: New models, successful applications},
  author={Holmes, John H and Lanzi, Pier Luca and Stolzmann, Wolfgang and Wilson, Stewart W},
  journal={Information Processing Letters},
  volume={82},
  number={1},
  pages={23--30},
  year={2002},
  publisher={Elsevier}
}

@article{holland1977cognitive,
  title={Cognitive systems based on adaptive algorithms},
  author={Holland, John H and Reitman, Judith S},
  journal={ACM SIGART Bulletin},
  number={63},
  pages={49--49},
  year={1977},
  publisher={ACM}
}

@article{booker1989classifier,
  title={Classifier systems and genetic algorithms},
  author={Booker, Lashon B. and Goldberg, David E. and Holland, John H.},
  journal={Artificial intelligence},
  volume={40},
  number={1},
  pages={235--282},
  year={1989},
  publisher={Elsevier}
}

@article{bacardit2009improving,
  title={Improving the scalability of rule-based evolutionary learning},
  author={Bacardit, Jaume and Burke, Edmund K and Krasnogor, Natalio},
  journal={Memetic Computing},
  volume={1},
  number={1},
  pages={55--67},
  year={2009},
  publisher={Springer}
}

@inproceedings{llora2007towards,
  title={Towards better than human capability in diagnosing prostate cancer using infrared spectroscopic imaging},
  author={Llor{\`a}, Xavier and Reddy, Rohith and Matesic, Brian and Bhargava, Rohit},
  booktitle={Proceedings of the 9th annual conference on Genetic and evolutionary computation},
  pages={2098--2105},
  year={2007},
  organization={ACM}
}

@inproceedings{hurst2004self,
  title={A self-adaptive neural learning classifier system with constructivism for mobile robot control},
  author={Hurst, Jacob and Bull, Larry},
  booktitle={Parallel Problem Solving from Nature-PPSN VIII},
  pages={942--951},
  year={2004},
  organization={Springer}
}


@inproceedings{butz2008context,
  title={Context-dependent predictions and cognitive arm control with XCSF},
  author={Butz, Martin V and Herbort, Oliver},
  booktitle={Proceedings of the 10th annual conference on Genetic and evolutionary computation},
  pages={1357--1364},
  year={2008},
  organization={ACM}
}


@inproceedings{van2009using,
  title={Using continuous action spaces to solve discrete problems},
  author={van Hasselt, Hado and Wiering, Marco A},
  booktitle={Neural Networks, 2009. IJCNN 2009. International Joint Conference on},
  pages={1149--1156},
  year={2009},
  organization={IEEE}
}

@inproceedings{lanzi2006classifier,
  title={Classifier prediction based on tile coding},
  author={Lanzi, Pier Luca and Loiacono, Daniele and Wilson, Stewart W and Goldberg, David E},
  booktitle={Proceedings of the 8th annual conference on Genetic and evolutionary computation},
  pages={1497--1504},
  year={2006},
  organization={ACM}
}

@article{whiteson2006evolutionary,
  title={Evolutionary function approximation for reinforcement learning},
  author={Whiteson, Shimon and Stone, Peter},
  journal={The Journal of Machine Learning Research},
  volume={7},
  pages={877--917},
  year={2006},
  publisher={JMLR. org}
}

@article{fritzke1995growing,
  title={A growing neural gas network learns topologies},
  author={Fritzke, Bernd},
  journal={Advances in neural information processing systems},
  volume={7},
  pages={625--632},
  year={1995},
  publisher={MORGAN KAUFMANN PUBLISHERS}
}

@book{kohonen2001self,
  title={Self-organizing maps},
  author={Kohonen, Teuvo},
  volume={30},
  year={2001},
  publisher={Springer}
}

@inproceedings{wiering2011reinforcement,
  title={Reinforcement learning algorithms for solving classification problems},
  author={Wiering, Marco A and van Hasselt, Hado and Pietersma, A-D and Schomaker, Lambert},
  booktitle={Adaptive Dynamic Programming And Reinforcement Learning (ADPRL), 2011 IEEE Symposium on},
  pages={91--96},
  year={2011},
  organization={IEEE}
}


@article{lehman2011abandoning,
  title={Abandoning objectives: Evolution through the search for novelty alone},
  author={Lehman, Joel and Stanley, Kenneth O},
  journal={Evolutionary computation},
  volume={19},
  number={2},
  pages={189--223},
  year={2011},
  publisher={MIT Press}
}

@inproceedings{reehuis2013novelty,
  title={Novelty and interestingness measures for design-space exploration},
  author={Reehuis, Edgar and Olhofer, Markus and Emmerich, Michael and Sendhoff, Bernhard and B{\"a}ck, Thomas},
  booktitle={Proceeding of the fifteenth annual conference on Genetic and evolutionary computation conference},
  pages={1541--1548},
  year={2013},
  organization={ACM}
}

@incollection{graening2010towards,
  title={Towards directed open-ended search by a novelty guided evolution strategy},
  author={Graening, Lars and Aulig, Nikola and Olhofer, Markus},
  booktitle={Parallel Problem Solving from Nature, PPSN XI},
  pages={71--80},
  year={2010},
  publisher={Springer}
}

@incollection{iqbal2012xcsr,
  title={XCSR with computed continuous action},
  author={Iqbal, Muhammad and Browne, Will N and Zhang, Mengjie},
  booktitle={AI 2012: Advances in Artificial Intelligence},
  pages={350--361},
  year={2012},
  publisher={Springer}
}

@article{lanzi2007generalization,
  title={Generalization in the {XCSF} classifier system: Analysis, improvement, and extension},
  author={Lanzi, P.L. and Loiacono, D. and Wilson, S.W. and Goldberg, D.E.},
  journal={Evolutionary Computation},
  volume={15},
  number={2},
  pages={133--168},
  year={2007},
  publisher={MIT Press}
}

@inproceedings{lanzi1997study,
  title={A Study of the Generalization Capabilities of {XCS}},
  author={Lanzi, P.L. and others},
  booktitle={Proceedings of the Seventh International Conference on Genetic Algorithm},
  pages={418--425},
  year={1997}
}

@inproceedings{Hutchinson1957,
  title={Concluding Remarks},
  author={Hutchinson, G.E.},
  booktitle={Cold Spring Harbor Symposia on Quantitative Biology 22},
  pages={415--427},
  year={1957}
}

@conference{vesterstrom2004comparative,
  title={{A comparative study of differential evolution, particle swarm optimization, and evolutionary algorithms on numerical benchmark problems}},
  author={Vesterstrom, J. and Thomsen, R.},
  booktitle={Evolutionary Computation, 2004. CEC2004. Congress on},
  volume={2},
  pages={1980--1987},
  isbn={0780385152},
  year={2004},
  organization={IEEE}
}

@article{butz2008function,
  title={Function approximation with {XCS}: Hyperellipsoidal conditions, recursive least squares, and compaction},
  author={Butz, M.V. and Lanzi, P.L. and Wilson, S.W.},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={12},
  number={3},
  pages={355--376},
  year={2008},
  publisher={IEEE}
}



@article{iorio2005solving,
  title={Solving rotated multi-objective optimization problems using differential evolution},
  author={Iorio, A. and Li, X.},
  journal={AI 2004: Advances in Artificial Intelligence},
  pages={861--872},
  year={2005},
  publisher={Springer}
}

@article{garcia2009study,
  title={{A study on the use of non-parametric tests for analyzing the evolutionary algorithms' behaviour: a case study on the CEC'2005 special session on real parameter optimization}},
  author={Garc{\'\i}a, S. and Molina, D. and Lozano, M. and Herrera, F.},
  journal={Journal of Heuristics},
  volume={15},
  number={6},
  pages={617--644},
  issn={1381-1231},
  year={2009},
  publisher={Springer}
}

@inproceedings{goldberg1987genetic,
  title={Genetic algorithms with sharing for multimodal function optimization},
  author={Goldberg, David E and Richardson, Jon},
  booktitle={Genetic algorithms and their applications: Proceedings of the Second International Conference on Genetic Algorithms},
  pages={41--49},
  year={1987},
  organization={Hillsdale, NJ: Lawrence Erlbaum}
}

@article{baranes2013active,
  title={Active learning of inverse models with intrinsically motivated goal exploration in robots},
  author={Baranes, Adrien and Oudeyer, Pierre-Yves},
  journal={Robotics and Autonomous Systems},
  volume={61},
  number={1},
  pages={49--73},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{urgen1991possibility,
  title={A possibility for implementing curiosity and boredom in model-building neural controllers},
  author={Schmidhuber, Jurgen},
  booktitle={From animals to animats: proceedings of the first international conference on simulation of adaptive behavior (SAB90)},
  year={1991},
  organization={Citeseer}
}

@article{schmidhuber2006developmental,
  title={Developmental robotics, optimal artificial curiosity, creativity, music, and the fine arts},
  author={Schmidhuber, J{\"u}rgen},
  journal={Connection Science},
  volume={18},
  number={2},
  pages={173--187},
  year={2006},
  publisher={Taylor \& Francis}
}

@article{oudeyer2007intrinsica,
  title={Intrinsic motivation systems for autonomous mental development},
  author={Oudeyer, Pierre-Yves and Kaplan, Fr{\'e}d{\'e}ric and Hafner, Verena V},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={11},
  number={2},
  pages={265--286},
  year={2007},
  publisher={IEEE}
}

@article{oudeyer2007intrinsic,
  title={What is intrinsic motivation? a typology of computational approaches},
  author={Oudeyer, Pierre-Yves and Kaplan, Frederic},
  journal={Frontiers in neurorobotics},
  volume={1},
  pages={6},
  year={2007},
  publisher={Frontiers}
}

@inproceedings{igel2000improving,
  title={Improving the Rprop learning algorithm},
  author={Igel, Christian and H{\"u}sken, Michael},
  booktitle={Proceedings of the second international ICSC symposium on neural computation (NC 2000)},
  volume={2000},
  pages={115--121},
  year={2000},
  organization={Citeseer}
}

@article{storn1997differential,
  title={{Differential evolution--a simple and efficient heuristic for global optimization over continuous spaces}},
  author={Storn, R. and Price, K.},
oarticle{storn1997differential,
  journal={Journal of global optimization},
  volume={11},
  number={4},
  pages={341--359},
  issn={0925-5001},
  year={1997},
  publisher={Springer}
}

@article{brest2006self,
  title={Self-adapting control parameters in differential evolution: A comparative study on numerical benchmark problems},
  author={Brest, J. and Greiner, S. and Boskovic, B. and Mernik, M. and Zumer, V.},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={10},
  number={6},
  pages={646--657},
  issn={1089-778X},
  year={2006},
  publisher={IEEE}
}

@inproceedings{belding1995distributed,
  title={The Distributed Genetic Algorithm Revisited},
  author={Belding, T.C.},
  booktitle={Proceedings of the Sixth International Conference on Genetic Algorithms: University of Pittsburgh, July 15-19, 1995},
  pages={114},
  year={1995},
  organization={Morgan Kaufmann Pub}
}

@INPROCEEDINGS{manderick1989,
AUTHOR = "Bernard Manderick and Piet Spiessens",
TITLE = "Fine-Grained Parallel Genetic Algorithms.",
booktitle = "ICGA'89",
PAGES = {428-433},
YEAR = {1989}  }

@inproceedings{howard2009towards,
  title={Towards continuous actions in continuous space and time using self-adaptive constructivism in neural {XCSF}},
  author={Howard, G.D. and Bull, L. and Lanzi, P.L.},
  booktitle={Proceedings of the 11th Annual conference on Genetic and evolutionary computation},
  pages={1219--1226},
  year={2009},
  organization={ACM}
}

@article{bonarini2000fuzzy,
  title={Fuzzy and crisp representations of real-valued input for learning classifier systems},
  author={Bonarini, A. and Bonacina, C. and Matteucci, M.},
  journal={Learning Classifier Systems},
  pages={107--124},
  year={2000},
  publisher={Springer}
}



@inproceedings{butz2008context,
  title={Context-dependent predictions and cognitive arm control with {XCSF}},
  author={Butz, M.V. and Herbort, O.},
  booktitle={Proceedings of the 10th annual conference on Genetic and evolutionary computation},
  pages={1357--1364},
  year={2008},
  organization={ACM}
}

@article{stalph2012learning,
  title={Learning local linear Jacobians for flexible and adaptive robot arm control},
  author={Stalph, P.O. and Butz, M.V.},
  journal={Genetic programming and evolvable machines},
  volume={13},
  number={2},
  pages={137--157},
  year={2012},
  publisher={Springer}
}

@inproceedings{tran2007xcsf,
  title={{XCSF} with computed continuous action},
  author={Tran, H.T. and Sanza, C. and Duthen, Y. and Nguyen, T.D.},
  booktitle={Genetic And Evolutionary Computation Conference: Proceedings of the 9 th annual conference on Genetic and evolutionary computation},
  volume={7},
  number={11},
  pages={1861--1869},
  year={2007}
}

@article{bull2002using,
  title={On using constructivism in neural classifier systems},
  author={Bull, L.},
  journal={Parallel problem solving from nature-PPSN VII},
  pages={558--567},
  year={2002},
  publisher={Springer}
}

@article{casillas2007fuzzy,
  title={{Fuzzy-XCS}: A Michigan genetic fuzzy system},
  author={Casillas, J. and Carse, B. and Bull, L.},
  journal={Fuzzy Systems, IEEE Transactions on},
  volume={15},
  number={4},
  pages={536--550},
  year={2007},
  publisher={IEEE}
}

@inproceedings{bull2002accuracy,
  title={Accuracy-based neuro and neuro-fuzzy classifier systems},
  author={Bull, L. and O'Hara, T.},
  booktitle={Proceedings of the Genetic and Evolutionary Computation Conference},
  pages={905--911},
  year={2002},
  organization={Morgan Kaufmann Publishers Inc.}
}

@inproceedings{lanzi2005xcs,
  title={{XCS} with computed prediction in multistep environments},
  author={Lanzi, P.L. and Loiacono, D. and Wilson, S.W. and Goldberg, D.E.},
  booktitle={Proceedings of the 2005 conference on Genetic and evolutionary computation},
  pages={1859--1866},
  year={2005},
  organization={ACM}
}

@inproceedings{valenzuela1991fuzzy,
  title={The fuzzy classifier system: A classifier system for continuously varying variables},
  author={Valenzuela-Rend{\'o}n, M.},
  booktitle={Proceedings of the Fourth International Conference on Genetic Algorithms pp346-353, Morgan Kaufmann I},
  volume={991},
  pages={223--230},
  year={1991}
}

@inproceedings{Widrow1960Adaptive,
    address = {New York},
    author = {Widrow, Bernard and Hoff, Marcian E.},
    booktitle = {1960 {IRE} {WESCON} Convention Record, Part 4},
    citeulike-article-id = {2510415},
    citeulike-linkout-0 = {http://isl-www.stanford.edu/\~{}widrow/papers/c1960adaptiveswitching.pdf},
    keywords = {neural-networks},
    pages = {96--104},
    posted-at = {2010-06-11 17:12:34},
    priority = {2},
    publisher = {{IRE}},
    title = {{Adaptive Switching Circuits}},
    url = {http://isl-www.stanford.edu/\~{}widrow/papers/c1960adaptiveswitching.pdf},
    year = {1960}
}

@article{mouret2011novelty,
  title={Novelty-based multiobjectivization},
  author={Mouret, J.B.},
  journal={New Horizons in Evolutionary Robotics},
  pages={139--154},
  year={2011},
  publisher={Springer}
}

@article{horn1994implicit,
  title={Implicit niching in a learning classifier system: Nature's way},
  author={Horn, J. and Goldberg, D.E. and Deb, K.},
  journal={Evolutionary Computation},
  volume={2},
  number={1},
  pages={37--66},
  year={1994},
  publisher={MIT Press}
}

@inproceedings{alba2000cellular,
  title={Cellular evolutionary algorithms: Evaluating the influence of ratio},
  author={Alba, E. and Troya, J.},
  booktitle={Parallel Problem Solving from Nature PPSN VI},
  pages={29--38},
  year={2000},
  organization={Springer}
}

@article{alba2002parallelism,
  title={Parallelism and evolutionary algorithms},
  author={Alba, E. and Tomassini, M.},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={6},
  number={5},
  pages={443--462},
  year={2002},
  publisher={IEEE}
}

@book{tomassini2005spatially,
  title={Spatially structured evolutionary algorithms},
  author={Tomassini, M.},
  year={2005},
  publisher={Springer}
}

@article{butz2004toward,
  title={Toward a theory of generalization and learning in {XCS}},
  author={Butz, M.V. and Kovacs, T. and Lanzi, P.L. and Wilson, S.W.},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={8},
  number={1},
  pages={28--46},
  year={2004},
  publisher={IEEE}
}

@article{butz2001algorithmic,
  title={An algorithmic description of {XCS}},
  author={Butz, M. and Wilson, S.},
  journal={Advances in Learning Classifier Systems},
  pages={267--274},
  year={2001},
  publisher={Springer}
}

@article{butz2001algorithmic,
  title={An algorithmic description of {XCS}},
  author={Butz, M. and Wilson, S.},
  journal={Advances in Learning Classifier Systems},
  pages={267--274},
  year={2001},
  publisher={Springer}
}

@article{wilson2002classifiers,
 author = {Wilson, Stewart W.},
 title = {Classifiers that approximate functions},
 issue_date = {June 2002},
 volume = {1},
 number = {2-3},
 month = jun,
 year = {2002},
 issn = {1567-7818},
 pages = {211--234},
 numpages = {24},
 url = {http://dx.doi.org/10.1023/A:1016535925043},
 doi = {10.1023/A:1016535925043},
 acmid = {599708},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
 keywords = {classifier systems, continuous actions, function approximation, generalized classifier},
} 

@article{kohonen1998self,
  title={The self-organizing map},
  author={Kohonen, T.},
  journal={Neurocomputing},
  volume={21},
  number={1},
  pages={1--6},
  year={1998},
  publisher={Elsevier}
}

@phdthesis{Booker:1982:IBA:910371,
 author = {Booker, Lashon Bernard},
 title = {Intelligent behavior as an adaptation to the task environment},
 year = {1982},
 note = {AAI8214966},
 publisher = {University of Michigan},
 address = {Ann Arbor, MI, USA},
} 

@article{wilson1995classifier,
  title={Classifier fitness based on accuracy},
  author={Wilson, S.W.},
  journal={Evolutionary computation},
  volume={3},
  number={2},
  pages={149--175},
  year={1995},
  publisher={MIT Press}
}

@article{lanzi2000roadmap,
  title={A roadmap to the last decade of learning classifier system research (from 1989 to 1999)},
  author={Lanzi, P. and Riolo, R.},
  journal={Learning Classifier Systems},
  pages={33--61},
  year={2000},
  publisher={Springer}
}

@article{urbanowicz2009learning,
  title={Learning classifier systems: a complete introduction, review, and roadmap},
  author={Urbanowicz, R.J. and Moore, J.H.},
  journal={Journal of Artificial Evolution and Applications},
  volume={2009},
  pages={1},
  year={2009},
  publisher={Hindawi Publishing Corp.}
}

@article{bacardit2006biohel,
  title={Biohel: Bioinformatics-oriented hierarchical evolutionary learning},
  author={Bacardit, J. and Krasnogor, N.},
  year={2006},
  publisher={Computer Science \& IT}
}

@inproceedings{llora2007towards,
  title={Towards better than human capability in diagnosing prostate cancer using infrared spectroscopic imaging},
  author={Llor{\`a}, X. and Reddy, R. and Matesic, B. and Bhargava, R.},
  booktitle={Proceedings of the 9th annual conference on Genetic and evolutionary computation},
  pages={2098--2105},
  year={2007},
  organization={ACM}
}

@ARTICLE{wilson1994zcs,
  TITLE= "{ZCS}: A zeroth level classifier system",
  author={Wilson, S.W.},
  journal={Evolutionary computation},
  volume={2},
  number={1},
  pages={1--18},
  year={1994},
  publisher={MIT Press}
}



@ARTICLE{bowman:reasoning,
	AUTHOR = "Mic Bowman and Saumya K. Debray and Larry L. Peterson",
	TITLE = "Reasoning About Naming Systems",
	JOURNAL = "ACM Trans. Program. Lang. Syst.",
	VOLUME = {15},
	NUMBER = {5},
	PAGES = {795-825},
	MONTH = "November",
	YEAR = {1993}	}

@ARTICLE{braams:babel,
	AUTHOR = "Johannes Braams",
	TITLE = "Babel, a Multilingual Style-Option System for Use with LaTeX's Standard Document Styles",
	JOURNAL = {TUGboat},
	VOLUME = {12},
	NUMBER = {2},
	PAGES = {291-301},
	MONTH = "June",
	YEAR = {1991}	}

@INPROCEEDINGS{clark:pct,
	AUTHOR = "Malcolm Clark",
	TITLE = "Post Congress Tristesse",
	BOOKTITLE = "TeX90 Conference Proceedings",
	PAGES = "84-89",
	ORGANIZATION = "TeX Users Group",
	MONTH = "March", 
	YEAR = {1991}	}

@ARTICLE{herlihy:methodology,
	AUTHOR = "Maurice Herlihy",
	TITLE = "A Methodology for Implementing Highly Concurrent
	Data Objects",
	JOURNAL = {ACM Trans. Program. Lang. Syst.},
	VOLUME = {15},
	NUMBER = {5},
	PAGES = {745-770},
	MONTH = "November",
	YEAR = {1993}	}

@BOOK{Lamport:LaTeX,
	AUTHOR = "Leslie Lamport",
	TITLE = "LaTeX User's Guide and Document Reference Manual",
	PUBLISHER = "Addison-Wesley Publishing Company",
	ADDRESS = "Reading, Massachusetts",
	YEAR = "1986"	}

@BOOK{salas:calculus,
	AUTHOR = "S.L. Salas and Einar Hille",
	TITLE = "Calculus: One and Several Variable",
	PUBLISHER = "John Wiley and Sons",
	ADDRESS = "New York",
	YEAR = "1978"	}






 @article{newman2003structure,
   title={The structure and function of complex networks},
   author={Newman, Mark EJ},
   journal={SIAM review},
   volume={45},
   number={2},
   pages={167--256},
   year={2003},
   publisher={SIAM}
 }
 
 @incollection{clune2007investigating,
   title={Investigating the emergence of phenotypic plasticity in evolving digital organisms},
   author={Clune, Jeff and Ofria, Charles and Pennock, Robert T},
   booktitle={Advances in Artificial Life},
   pages={74--83},
   year={2007},
   publisher={Springer}
 }
 


 @inproceedings{lessin2013open,
   title={Open-ended behavioral complexity for evolved virtual creatures},
   author={Lessin, Dan and Fussell, Don and Miikkulainen, Risto},
   booktitle={Proceeding of the fifteenth annual conference on Genetic and evolutionary computation conference},
   pages={335--342},
   year={2013},
   organization={ACM}
 }



 @article{lehman2011abandoning,
   title={Abandoning objectives: Evolution through the search for novelty alone},
   author={Lehman, Joel and Stanley, Kenneth O},
   journal={Evolutionary computation},
   volume={19},
   number={2},
   pages={189--223},
   year={2011},
   publisher={MIT Press}
 }
 
 @inproceedings{kawai2001incremental,
   title={Incremental evolution of neurocontrollers with a diffusion-reaction mechanism of neuromodulators},
   author={Kawai, Katsumi and Ishiguro, Akio and Eggenberger, Peter},
   booktitle={Intelligent Robots and Systems, 2001. Proceedings. 2001 IEEE/RSJ International Conference on},
   volume={4},
   pages={2384--2391},
   year={2001},
   organization={IEEE}
 }
 
 @article{nelson2009fitness,
   title={Fitness functions in evolutionary robotics: A survey and analysis},
   author={Nelson, Andrew L and Barlow, Gregory J and Doitsidis, Lefteris},
   journal={Robotics and Autonomous Systems},
   volume={57},
   number={4},
   pages={345--370},
   year={2009},
   publisher={Elsevier}
 }
 
 @article{kondo2007evolutionary,
   title={Evolutionary design and behavior analysis of neuromodulatory neural networks for mobile robots control},
   author={Kondo, Toshiyuki},
   journal={Applied Soft Computing},
   volume={7},
   number={1},
   pages={189--202},
   year={2007},
   publisher={Elsevier}
 }
 
 @article{niv2002evolution,
   title={Evolution of reinforcement learning in uncertain environments: A simple explanation for complex foraging behaviors},
   author={Niv, Yael and Joel, Daphna and Meilijson, Isaac and Ruppin, Eytan},
   journal={Adaptive Behavior},
   volume={10},
   number={1},
   pages={5--24},
   year={2002},
   publisher={Sage Publications}
 }
 
 @inproceedings{risi2009novelty,
   title={How novelty search escapes the deceptive trap of learning to learn},
   author={Risi, Sebastian and Vanderbleek, Sandy D and Hughes, Charles E and Stanley, Kenneth O},
   booktitle={Proceedings of the 11th Annual conference on Genetic and evolutionary computation},
   pages={153--160},
   year={2009},
   organization={ACM}
 }
 
 @inproceedings{soltoggio2008evolutionary,
   title={Evolutionary Advantages of Neuromodulated Plasticity in Dynamic, Reward-based Scenarios.},
   author={Soltoggio, Andrea and Bullinaria, John A and Mattiussi, Claudio and D{\"u}rr, Peter and Floreano, Dario},
   booktitle={ALIFE},
   pages={569--576},
   year={2008}
 }
 
 @inproceedings{soltoggio2007evolving,
   title={Evolving neuromodulatory topologies for reinforcement learning-like problems},
   author={Soltoggio, Andrea and Durr, P and Mattiussi, Claudio and Floreano, Dario},
   booktitle={Evolutionary Computation, 2007. CEC 2007. IEEE Congress on},
   pages={2471--2478},
   year={2007},
   organization={IEEE}
 }
 
 @incollection{mouret2014artificial,
   title={Artificial evolution of plastic neural networks: a few key concepts},
   author={Mouret, Jean-Baptiste and Tonelli, Paul},
   booktitle={Growing Adaptive Machines},
   pages={251--261},
   year={2014},
   publisher={Springer}
 }
 
 @article{marder2002cellular,
   title={Cellular, synaptic and network effects of neuromodulation},
   author={Marder, Eve and Thirumalai, Vatsala},
   journal={Neural Networks},
   volume={15},
   number={4},
   pages={479--493},
   year={2002},
   publisher={Elsevier}
 }
 
 @article{urzelai2001evolution,
   title={Evolution of adaptive synapses: Robots with fast adaptive behavior in new environments},
   author={Urzelai, Joseba and Floreano, Dario},
   journal={Evolutionary computation},
   volume={9},
   number={4},
   pages={495--524},
   year={2001},
   publisher={MIT Press}
 }
 
 @inproceedings{stanley2003evolving,
   title={Evolving adaptive neural networks with and without adaptive synapses},
   author={Stanley, Kenneth O and Bryant, Bobby D and Miikkulainen, Risto},
   booktitle={Evolutionary Computation, 2003. CEC'03. The 2003 Congress on},
   volume={4},
   pages={2557--2564},
   year={2003},
   organization={IEEE}
 }



 @book{kandel2012principles,
   title={Principles of neural science},
   author={Kandel, Eric R and Schwartz, James H and Jessell, Thomas M and Siegelbaum, Steven and Hudspeth, A. J.},
   volume={5},
   year={2012},
   publisher={McGraw-Hill New York}
 }
 
 @article{kohonen1990self,
   title={The self-organizing map},
   author={Kohonen, Teuvo},
   journal={Proceedings of the IEEE},
   volume={78},
   number={9},
   pages={1464--1480},
   year={1990},
   publisher={IEEE}
 }
 
 @article{sirat1990neural,
   title={Neural trees: a new tool for classification},
   author={Sirat, JA and Nadal, JP},
   journal={Network: Computation in Neural Systems},
   volume={1},
   number={4},
   pages={423--438},
   year={1990},
   publisher={Informa UK Ltd UK}
 }
 
 @article{golea1990growth,
   title={A growth algorithm for neural network decision trees},
   author={Golea, Mostefa and Marchand, Mario},
   journal={EPL (Europhysics Letters)},
   volume={12},
   number={3},
   pages={205},
   year={1990},
   publisher={IOP Publishing}
 }
 
 @article{paine2005hierarchical,
   title={How hierarchical control self-organizes in artificial adaptive systems},
   author={Paine, Rainer W and Tani, Jun},
   journal={Adaptive Behavior},
   volume={13},
   number={3},
   pages={211--225},
   year={2005},
   publisher={Sage Publications}
 }
 
 @article{murthy1998automatic,
   title={Automatic construction of decision trees from data: A multi-disciplinary survey},
   author={Murthy, Sreerama K},
   journal={Data mining and knowledge discovery},
   volume={2},
   number={4},
   pages={345--389},
   year={1998},
   publisher={Springer}
 }
 
 @article{precup1998multi,
   title={Multi-time models for temporally abstract planning},
   author={Precup, Doina and Sutton, Richard S},
   journal={Advances in neural information processing systems},
   pages={1050--1056},
   year={1998},
   publisher={MORGAN KAUFMANN PUBLISHERS}
 }
 
 
 @article{nolfi2002evolving,
   title={Evolving robots able to self-localize in the environment: the importance of viewing cognition as the result of processes occurring at different time-scales},
   author={Nolfi, Stefano},
   journal={Connection Science},
   volume={14},
   number={3},
   pages={231--244},
   year={2002},
   publisher={Taylor \& Francis}
 }
 
 @article{kiebel2008hierarchy,
   title={A hierarchy of time-scales and the brain},
   author={Kiebel, Stefan J and Daunizeau, Jean and Friston, Karl J},
   journal={PLoS computational biology},
   volume={4},
   number={11},
   pages={e1000209},
   year={2008},
   publisher={Public Library of Science}
 }
 
 @book{levitan2002neuron,
   title={The neuron: cell and molecular biology},
   author={Levitan, Irwin B and Kaczmarek, Leonard K},
   year={2002},
   publisher={Oxford University Press}
 }
 
 @article{grossberg1982studies,
   title={Studies of mind and brain},
   author={Grossberg, Stephen},
   journal={Reidel, Boston},
   pages={5--213},
   year={1982}
 }
 
 @article{lecun1998gradient,
   title={Gradient-based learning applied to document recognition},
   author={LeCun, Y. and Bottou, L. and Bengio, Y. and Haffner, P.},
   journal={Proceedings of the IEEE},
   volume={86},
   number={11},
   pages={2278--2324},
   year={1998},
   publisher={IEEE}
 }
 
 @book{hastie2009elements,
   title={{The elements of statistical learning: data mining, inference, and prediction}},
   author={Hastie, T. and Tibshirani, R. and Friedman, J.H.},
   year={2009},
   publisher={Springer Verlag}
 }
 
 @book{laughlin2006different,
   title={A different universe: Reinventing physics from the bottom down},
   author={Laughlin, R.B.},
   year={2006},
   publisher={Basic Books}
 }
 
 @book{ryle2002concept,
   title={The concept of mind},
   author={Ryle, G.},
   year={2002},
   publisher={University of Chicago Press}
 }
 
 @article{kraskov2008,
   title={{Synchronization and Interdependence Measures and Their Application to the Electroencephalogram of Epilepsy Patients and Clustering of Data}},
   author={Kraskov, A.},
   journal={Report Nr.: NIC series; 24},
   year={2008}
 }
 
 @article{kraskov2003,
   title={{Hierarchical clustering based on mutual information}},
   author={Kraskov, A. and St\"{o}gbauer, H. and Andrzejak, R.G. and Grassberger, P.},
   journal={Arxiv preprint q-bio/0311039},
   year={2003}
 }
 
 @article{dionisio2006,
   title={{Entropy-based independence test}},
   author={Dion{\'\i}sio, A. and Menezes, R. and Mendes, D.A.},
   journal={Nonlinear Dynamics},
   volume={44},
   number={1},
   pages={351--357},
   year={2006},
   publisher={Springer}
 }
 
 @conference{aghagolzadeh2007,
   title={{A hierarchical clustering based on mutual information maximization}},
   author={Aghagolzadeh, M. and Soltanian-Zadeh, H. and Araabi, B. and Aghagolzadeh, A.},
   booktitle={IEEE International Conference on Image Processing, 2007. ICIP 2007},
   volume={1},
   year={2007},
   organization={Citeseer}
 }
 
 @conference{aporntewan2009,
   title={{Gene hunting of the Genetic Analysis Workshop 16 rheumatoid arthritis data using rough set theory}},
   author={Aporntewan, C. and Ballard, D. and Lee, J. and Lee, J. and Wu, Z. and Zhao, H.},
   booktitle={BMC proceedings},
   volume={3},
   number={Suppl 7},
   pages={S126},
   year={2009},
   organization={BioMed Central Ltd}
 }
 
 @article{kerschen2004feature,
   title={Feature extraction using auto-associative neural networks},
   author={Kerschen, G. and Golinval, J.C.},
   journal={Smart materials and structures},
   volume={13},
   pages={211},
   year={2004},
   publisher={IOP Publishing}
 }
 
 @article{bengio2005curse,
   title={The curse of dimensionality for local kernel machines},
   author={Bengio, Y. and Delalleau, O. and Le Roux, N.},
   journal={Techn. Rep},
   volume={1258},
   year={2005},
   publisher={Citeseer}
 }
 
 @article{shannon1948,
   title={A mathematical theory of communication},
   author={Shannon, C.},
   journal={Bell System Technical Journal},
   volume={27},
   number={10},
   pages={623--656},
   year={1948}
 }
 
 @inproceedings{bengio2006non,
   title={Non-local manifold parzen windows},
   author={Bengio, Y. and Larochelle, H. and Vincent, P.},
   booktitle={In Advances in Neural Information Processing Systems 18},
   year={2006}
 }
 
 @article{håstad1991power,
   title={On the power of small-depth threshold circuits},
   author={H{\aa}stad, J. and Goldmann, M.},
   journal={Computational Complexity},
   volume={1},
   number={2},
   pages={113--129},
   year={1991},
   publisher={Springer}
 }
 
 @article{bengio2009learning,
   title={Learning deep architectures for AI},
   author={Bengio, Y.},
   journal={Foundations and Trends{\textregistered} in Machine Learning},
   volume={2},
   number={1},
   pages={1--127},
   year={2009},
   publisher={Now Publishers Inc.}
 }
 
 
 @article{hinton2006fast,
   title={A fast learning algorithm for deep belief nets},
   author={Hinton, G.E. and Osindero, S. and Teh, Y.W.},
   journal={Neural computation},
   volume={18},
   number={7},
   pages={1527--1554},
   year={2006},
   publisher={MIT Press}
 }
 
 
 @article{bengio2007scaling,
   title={Scaling learning algorithms towards AI},
   author={Bengio, Y. and LeCun, Y.},
   journal={Large-Scale Kernel Machines},
   volume={1},
   pages={1--41},
   year={2007},
   publisher={Citeseer}
 }
 
 @article{cover1965geometrical,
   title={Geometrical and statistical properties of systems of linear inequalities with applications in pattern recognition},
   author={Cover, T.M.},
   journal={Electronic Computers, IEEE Transactions on},
   number={3},
   pages={326--334},
   year={1965},
   publisher={IEEE}
 }
 
 @article{gottlieb1984,
 	title = "Evolutionary trends and evolutionary origins: Relevance to theory in comparative psychology",
 	journal = "Psychological Review",
 	volume = "91",
 	number = "4",
 	pages = "448 - 456",
 	year = "1984",
 	note = "",
 	issn = "0033-295X",
 	doi = "DOI: 10.1037/0033-295X.91.4.448",
 	author = "Gilbert Gottlieb",
 	keywords = "evolutionary trends & origins & comparative psychology theory"
 }
 
 @article{smith1999learning,
   title={Learning theory},
   author={Smith, MK},
   journal={The encyclopedia of informal education},
   note={\url{www.infed.org/biblio/b-learn.htm}; accessed September 12, 2011.},
   year={1999}
 }
 
 
 @book{rogers2003difference,
   title={What is the difference?: a new critique of adult learning and teaching},
   author={Rogers, A.},
   year={2003},
   publisher={NIACE Leicester}
 }
 
 @book{rogers1969freedom,
   title={Freedom to learn: A view of what education might become},
   author={Rogers, C.R.},
   year={1969},
   publisher={CE Merrill Pub. Co.(Columbus, Ohio)}
 }
 
 @article{back2002evolutionary,
   title={{Evolutionary computation: Comments on the history and current state}},
   author={Back, T. and Hammel, U. and Schwefel, H.P.},
   journal={Evolutionary Computation, IEEE Transactions on},
   volume={1},
   number={1},
   pages={3--17},
   issn={1089-778X},
   year={2002},
   publisher={IEEE}
 }
 
 @book{friedenberg2005cognitive,
   title={{Cognitive science: An introduction to the study of mind}},
   author={Friedenberg, J. and Silverman, G.},
   isbn={1412925681},
   pages={85--88},
   year={2005},
   publisher={Sage Publications, Inc}
 }
 
 @article{black2002black,
   title={{Black-box analysis of the block-cipher-based hash-function constructions from PGV}},
   author={Black, J. and Rogaway, P. and Shrimpton, T.},
   journal={Advances in Cryptology-CRYPTO 2002},
   pages={103--118},
   year={2002},
   publisher={Springer}
 }
 
 @book{cauer1954theorie,
   title={{Theorie der linearen Wechselstromschaltungen}},
   author={Cauer, W.},
   year={1954},
   publisher={Akademie-Verlag}
 }
 
 @book{goldberg2002,
   title={{The design of innovation: Lessons from and for competent genetic algorithms}},
   author={Goldberg, D.E.},
   year={2002},
   publisher={Springer}
 }
 
 @article{kirkpatrick1984optimization,
   title={{Optimization by simulated annealing: Quantitative studies}},
   author={Kirkpatrick, S.},
   journal={Journal of Statistical Physics},
   volume={34},
   number={5},
   pages={975--986},
   issn={0022-4715},
   year={1984},
   publisher={Springer}
 }
 
 @article{poli2009there,
   title={{There is a free lunch for hyper-heuristics, genetic programming and computer scientists}},
   author={Poli, R. and Graff, M.},
   journal={Genetic Programming},
   pages={195--207},
   year={2009},
   publisher={Springer}
 }
 
 @article{hruschka2006evolving,
   title={{Evolving clusters in gene-expression data}},
   author={Hruschka, E.R. and Campello, R.J.G.B. and De Castro, L.N.},
   journal={Information Sciences},
   volume={176},
   number={13},
   pages={1898--1927},
   issn={0020-0255},
   year={2006},
   publisher={Elsevier}
 }
 
 @article{kicinger2005evolutionary,
   title={{Evolutionary computation and structural design: A survey of the state-of-the-art}},
   author={Kicinger, R. and Arciszewski, T. and Jong, K.D.},
   journal={Computers \& Structures},
   volume={83},
   number={23-24},
   pages={1943--1978},
   issn={0045-7949},
   year={2005},
   publisher={Elsevier}
 }
 
 
 @book{darwin2003origin,
   title={{The origin of species}},
   author={Darwin, C.},
   isbn={0451529065},
   year={2003},
   publisher={Signet Classic}
 }
 
 @article{storn1997differential,
   title={{Differential evolution--a simple and efficient heuristic for global optimization over continuous spaces}},
   author={Storn, R. and Price, K.},
   journal={Journal of global optimization},
   volume={11},
   number={4},
   pages={341--359},
   issn={0925-5001},
   year={1997},
   publisher={Springer}
 }
 
 @conference{vesterstrom2004comparative,
   title={{A comparative study of differential evolution, particle swarm optimization, and evolutionary algorithms on numerical benchmark problems}},
   author={Vesterstrom, J. and Thomsen, R.},
   booktitle={Evolutionary Computation, 2004. CEC2004. Congress on},
   volume={2},
   pages={1980--1987},
   isbn={0780385152},
   year={2004},
   organization={IEEE}
 }
 
 @article{liu2005fuzzy,
   title={{A fuzzy adaptive differential evolution algorithm}},
   author={Liu, J. and Lampinen, J.},
   journal={Soft Computing-A Fusion of Foundations, Methodologies and Applications},
   volume={9},
   number={6},
   pages={448--462},
   issn={1432-7643},
   year={2005},
   publisher={Springer}
 }
 
 @conference{slowik2008training,
   title={{Training of artificial neural networks using differential evolution algorithm}},
   author={Slowik, A. and Bialko, M.},
   booktitle={Human System Interactions, 2008 Conference on},
   pages={60--65},
   year={2008},
   organization={IEEE}
 }
 
 @article{levenberg1944method,
   title={{A method for the solution of certain nonlinear problems in least squares}},
   author={Levenberg, K.},
   journal={Quart. Appl. Math},
   volume={2},
   number={2},
   pages={164--168},
   year={1944}
 }
 
 @article{halkidi2001clustering,
   title={{On clustering validation techniques}},
   author={Halkidi, M. and Batistakis, Y. and Vazirgiannis, M.},
   journal={Journal of Intelligent Information Systems},
   volume={17},
   number={2},
   pages={107--145},
   issn={0925-9902},
   year={2001},
   publisher={Springer}
 }
 
 @article{jain1999data,
   title={{Data clustering: a review}},
   author={Jain, A.K. and Murty, M.N. and Flynn, P.J.},
   journal={ACM computing surveys (CSUR)},
   volume={31},
   number={3},
   pages={264--323},
   issn={0360-0300},
   year={1999},
   publisher={ACM}
 }
 
 @article{campello2009efficiency,
   title={{On the efficiency of evolutionary fuzzy clustering}},
   author={Campello, R.J.G.B. and Hruschka, E.R. and Alves, V.S.},
   journal={Journal of Heuristics},
   volume={15},
   number={1},
   pages={43--75},
   issn={1381-1231},
   year={2009},
   publisher={Springer}
 }
 
 @article{rousseeuw1987silhouettes,
   title={{Silhouettes: a graphical aid to the interpretation and validation of cluster analysis}},
   author={Rousseeuw, P.J.},
   journal={Journal of computational and applied mathematics},
   volume={20},
   pages={53--65},
   issn={0377-0427},
   year={1987},
   publisher={Elsevier}
 }
 
 @article{sharp1968cardinality,
   title={{Cardinality of finite topologies*}},
   author={Sharp Jr, H.},
   journal={Journal of Combinatorial Theory},
   volume={5},
   number={1},
   pages={82--86},
   issn={0021-9800},
   year={1968},
   publisher={Elsevier}
 }
 
 @article{ruspini1970numerical,
   title={{Numerical methods for fuzzy clustering}},
   author={Ruspini, E.H.},
   journal={Information Sciences},
   volume={2},
   number={3},
   pages={319--350},
   issn={0020-0255},
   year={1970},
   publisher={Elsevier}
 }
 
 @article{ho2002simple,
   title={{Simple explanation of the no-free-lunch theorem and its implications}},
   author={Ho, Y.C. and Pepyne, D.L.},
   journal={Journal of Optimization Theory and Applications},
   volume={115},
   number={3},
   pages={549--570},
   issn={0022-3239},
   year={2002},
   publisher={Springer}
 }
 
 @conference{ewert2009evolutionary,
   title={{Evolutionary synthesis of nand logic: Dissecting a digital organism}},
   author={Ewert, W. and Dembski, W.A. and Marks, RJ},
   booktitle={Systems, Man and Cybernetics, 2009. SMC 2009. IEEE International Conference on},
   pages={3047--3053},
   issn={1062-922X},
   year={2009},
   organization={IEEE}
 }
 
 @article{droste1998perhaps,
   title={{Perhaps not a free lunch but at least a free appetizer}},
   author={Droste, S. and Jansen, T. and Wegener, I.},
   journal={HT014601767},
   year={1998},
   publisher={Unversit{\\"a}t Dortmund}
 }
 
 @INPROCEEDINGS{whitley1999afree,
     author = {D. Whitley},
     title = {A Free Lunch Proof for Gray versus Binary Encodings},
     booktitle = {In},
     year = {1999},
     pages = {726--733},
     publisher = {Morgan Kaufmann}
 }
 
 @article{igel2001classes,
   title={{On classes of functions for which no free lunch results hold}},
   author={Igel, C. and Toussaint, M.},
   journal={Arxiv preprint cs/0108011},
   year={2001}
 }
 
 @conference{schumacher2001no,
   title={{The no free lunch and problem description length}},
   author={Schumacher, C. and Vose, MD and Whitley, LD},
   booktitle={Proceedings of the Genetic and Evolutionary Computation Conference (GECCO-2001)},
   pages={565--570},
   year={2001},
   organization={Citeseer}
 }
 
 @conference{lima2008investigating,
   title={{Investigating restricted tournament replacement in ECGA for non-stationary environments}},
   author={Lima, C.F. and Fernandes, C. and Lobo, F.G.},
   booktitle={Proceedings of the 10th annual conference on Genetic and evolutionary computation},
   pages={439--446},
   year={2008},
   organization={ACM}
 }
 
 @techreport{wolpert1995nfl,
     author = {David H. Wolpert and William G.},
     title = {No Free Lunch Theorems for Search},
     institution={The Santa Fe Institute},
     year = {1995}
 }
 
 @article{wolpert1997nfl,
   title={{No Free Lunch Theorems for Optimization}},
   author={Wolpert, D.H. and Macready, W.G.},
   journal={Evolutionary Computation, IEEE Transactions on},
   volume={1},
   number={1},
   pages={67--82},
   issn={1089-778X},
   year={1997},
   publisher={IEEE}
 }
 
 @conference{jin2006alleviating,
   title={{Alleviating catastrophic forgetting via multi-objective learning}},
   author={Jin, Y. and Sendhoff, B.},
   booktitle={Neural Networks, 2006. IJCNN'06. International Joint Conference on},
   pages={3335--3342},
   isbn={0780394909},
   year={2006},
   organization={IEEE}
 }
 
 @article{wolpert2005coevolutionary,
   title={{Coevolutionary free lunches}},
   author={Wolpert, D.H. and Macready, W.G.},
   journal={Evolutionary Computation, IEEE Transactions on},
   volume={9},
   number={6},
   pages={721--735},
   issn={1089-778X},
   year={2005},
   publisher={IEEE}
 }
 
 @conference{ester1996density,
   title={{A density-based algorithm for discovering clusters in large spatial databases with noise}},
   author={Ester, M. and Kriegel, H.P. and Sander, J. and Xu, X.},
   booktitle={Proc. KDD},
   volume={96},
   pages={226--231},
   year={1996}
 }
 
 @article{zhou2006fuzzy,
   title={Fuzzy causal networks: General model, inference, and convergence},
   author={Zhou, S. and Liu, Z.Q. and Zhang, J.Y.},
   journal={Fuzzy Systems, IEEE Transactions on},
   volume={14},
   number={3},
   pages={412--420},
   year={2006},
   publisher={IEEE}
 }
 
 @article{petalas2009improving,
   title={Improving fuzzy cognitive maps learning through memetic particle swarm optimization},
   author={Petalas, YG and Parsopoulos, KE and Vrahatis, MN},
   journal={Soft Computing-A Fusion of Foundations, Methodologies and Applications},
   volume={13},
   number={1},
   pages={77--94},
   year={2009},
   publisher={Springer}
 }
 
 @article{kosko1986fuzzy,
   title={Fuzzy cognitive maps},
   author={Kosko, B.},
   journal={International Journal of Man-Machine Studies},
   volume={24},
   number={1},
   pages={65--75},
   year={1986},
   publisher={Elsevier}
 }
 
 @article{zhi2001causation,
   title={Causation, bayesian networks, and cognitive maps},
   author={Zhi-Qiang, LIU},
   journal={Acta automatica sinica},
   volume={27},
   number={4},
   pages={552--566},
   year={2001}
 }
 
 @article{stach2005genetic,
   title={Genetic learning of fuzzy cognitive maps},
   author={Stach, W. and Kurgan, L. and Pedrycz, W. and Reformat, M.},
   journal={Fuzzy sets and systems},
   volume={153},
   number={3},
   pages={371--401},
   year={2005},
   publisher={Elsevier North-Holland, Inc.}
 }
 
 @article{harwood2002genetic,
   title={Genetic algorithm search over causal models},
   author={Harwood, S. and Scheines, R.},
   year={2002}
 }
 
 @book{papoulis1965probability,
   title={Probability, random variables, and stochastic processes},
   author={Papoulis, A. and Pillai, S.U. and Unnikrishna, S.},
   volume={196},
   year={1965},
   publisher={McGraw-hill New York}
 }
 
 @book{cover1991elements,
   title={Elements of information theory},
   author={Cover, T.M. and Thomas, J.A. and MyiLibrary},
   volume={6},
   year={1991},
   publisher={Wiley Online Library}
 }
 
 @article{kriegel2009clustering,
   title={{Clustering high-dimensional data: A survey on subspace clustering, pattern-based clustering, and correlation clustering}},
   author={Kriegel, H.P. and Kr\"{o}ger, P. and Zimek, A.},
   journal={ACM Transactions on Knowledge Discovery from Data (TKDD)},
   volume={3},
   number={1},
   pages={1--58},
   issn={1556-4681},
   year={2009},
   publisher={ACM}
 }
 
 @conference{mukhopadhyay2008multiobjective,
   title={{Multiobjective genetic fuzzy clustering of categorical attributes}},
   author={Mukhopadhyay, A. and Maulik, U. and Bandyopadhyay, S.},
   booktitle={Information Technology,(ICIT 2007). 10th International Conference on},
   pages={74--79},
   isbn={0769530680},
   year={2008},
   organization={IEEE}
 }
 
 @article{korkmaz2010multi,
   title={{Multi-objective Genetic Algorithms for grouping problems}},
   author={Korkmaz, E.E.},
   journal={Applied Intelligence},
   pages={1--14},
   issn={0924-669X},
   year={2010},
   publisher={Springer}
 }
 
 @article{du2005alternative,
   title={{Alternative clustering by utilizing multi-objective genetic algorithm with linked-list based chromosome encoding}},
   author={Du, J. and Korkmaz, E.E. and Alhajj, R. and Barker, K.},
   journal={Machine Learning and Data Mining in Pattern Recognition},
   pages={346--355},
   year={2005},
   publisher={Springer}
 }
 
 @article{dunn1973fuzzy,
   title={{A fuzzy relative of the ISODATA process and its use in detecting compact well-separated clusters}},
   author={Dunn, JC},
   journal={Cybernetics and Systems},
   volume={3},
   number={3},
   pages={32--57},
   issn={0196-9722},
   year={1973},
   publisher={Taylor \& Francis}
 }
 
 @article{bezdek1974numerical,
   title={{Numerical taxonomy with fuzzy sets}},
   author={Bezdek, J.C.},
   journal={Journal of Mathematical Biology},
   volume={1},
   number={1},
   pages={57--71},
   issn={0303-6812},
   year={1974},
   publisher={Springer}
 }
 
 
 @article{bandyopadhyay2007multiobjective,
   title={{Multiobjective genetic clustering for pixel classification in remote sensing imagery}},
   author={Bandyopadhyay, S. and Maulik, U. and Mukhopadhyay, A.},
   journal={Geoscience and Remote Sensing, IEEE Transactions on},
   volume={45},
   number={5},
   pages={1506--1511},
   issn={0196-2892},
   year={2007},
   publisher={IEEE}
 }
 
 
 @article{garcia2009study,
   title={{A study on the use of non-parametric tests for analyzing the evolutionary algorithms' behaviour: a case study on the CEC'2005 special session on real parameter optimization}},
   author={Garc{\'\i}a, S. and Molina, D. and Lozano, M. and Herrera, F.},
   journal={Journal of Heuristics},
   volume={15},
   number={6},
   pages={617--644},
   issn={1381-1231},
   year={2009},
   publisher={Springer}
 }
 
 
 @article{vendramin2010relative,
   title={{Relative clustering validity criteria: A comparative overview}},
   author={Vendramin, L. and Campello, R.J.G.B. and Hruschka, E.R.},
   journal={Statistical Analysis and Data Mining},
   volume={3},
   number={4},
   pages={209--235},
   issn={1932-1872},
   year={2010},
   publisher={Wiley Online Library}
 }
 
 
 @article{ilonen2003differential,
   title={{Differential evolution training algorithm for feed-forward neural networks}},
   author={Ilonen, J. and Kamarainen, J.K. and Lampinen, J.},
   journal={Neural Processing Letters},
   volume={17},
   number={1},
   pages={93--105},
   issn={1370-4621},
   year={2003},
   publisher={Springer}
 }
 
 
 @article{brest2006self,
   title={{Self-adapting control parameters in differential evolution: A comparative study on numerical benchmark problems}},
   author={Brest, J. and Greiner, S. and Boskovic, B. and Mernik, M. and Zumer, V.},
   journal={Evolutionary Computation, IEEE Transactions on},
   volume={10},
   number={6},
   pages={646--657},
   issn={1089-778X},
   year={2006},
   publisher={IEEE}
 }
 
 
 @conference{storn2002minimizing,
   title={{Minimizing the real functions of the ICEC'96 contest by differential evolution}},
   author={Storn, R. and Price, K.},
   booktitle={Evolutionary Computation, 1996., Proceedings of IEEE International Conference on},
   pages={842--844},
   isbn={0780329023},
   year={2002},
   organization={IEEE}
 }
 
 
 @book{rojas1996neural,
   title={{Neural networks: a systematic introduction}},
   author={Rojas, R.},
   year={1996},
   publisher={Springer}
 }
 
 @article{sprecher1965structure,
   title={{On the Structure of Continuous Functions of Several Variables}},
   author={Sprecher, D.A.},
   journal={Transactions of the American Mathematical Society},
   volume={115},
   pages={340--355},
   issn={0002-9947},
   year={1965},
   publisher={JSTOR}
 }
 
 @article{kolmogorov1957continuous,
   title={{On the representation of continuous functions of several variables as superpositions of continuous functions of a smaller number of variables}},
   author={Kolmogorov, A.N.},
   journal={Doklady Akademii Nauk SSSR},
   volume={104},
   pages={679--681},
   year={1957},
   publisher={American Mathematical Society.},
   note={(in Russian)}
 }
 
 @article{rosenblatt1958perceptron,
   title={{The perceptron: A probabilistic model for information storage and organization in the brain}},
   author={Rosenblatt, F.},
   journal={Psychological review},
   volume={65},
   number={6},
   pages={386--408},
   year={1958}
 }
 
 @book{slotine1991applied,
   title={{Applied nonlinear control}},
   author={Slotine, J.J.E. and Li, W. and others},
   year={1991},
   publisher={Prentice hall Englewood Cliffs, NJ}
 }
 
 @techreport{hand1999non,
   title={{Non-Linear and Linear Model Based Controller Design for Variable-Speed Wind Turbines}},
   author={Hand, MM and Balas, MJ},
   year={1999},
   institution={National Renewable Energy Lab., Golden, CO (US)}
 }
 


%----------------------- Cryptography with Optimization --------------------------


@article{sindhuja2014symmetric,
	title={A symmetric key encryption technique using genetic algorithm},
	author={Sindhuja, K},
	publisher={Citeseer}
}

@inproceedings{abd2011known,
  title={Known-plaintext attack of DES-16 using Particle Swarm Optimization},
  author={Abd-Elmonim, Wafaa G and Ghali, Neveen I and Hassanien, Aboul Ella and Abraham, Ajith},
  booktitle={Nature and Biologically Inspired Computing (NaBIC), 2011 Third World Congress on},
  pages={12--16},
  year={2011},
  organization={IEEE}
}


 


==> unused2 <==

@incollection{clune2007investigating,
  title={Investigating the emergence of phenotypic plasticity in evolving digital organisms},
  author={Clune, Jeff and Ofria, Charles and Pennock, Robert T},
  booktitle={Advances in Artificial Life},
  pages={74--83},
  year={2007},
  publisher={Springer}
}

@article{hornik1989multilayer,
  title={Multilayer feedforward networks are universal approximators},
  author={Hornik, Kurt and Stinchcombe, Maxwell and White, Halbert},
  journal={Neural networks},
  volume={2},
  number={5},
  pages={359--366},
  year={1989},
  publisher={Elsevier}
}

@PhdThesis{gruau1994neural,
  title={Neural Network Synthesis using Cellular Encoding and the Genetic Algorithm.},
  author={Gruau, Frederic and others},
  year={1994},
  school={Ecole Normale Superieure de Lyon}
}


@article{moriarty1997forming,
  title={Forming neural networks through efficient and adaptive coevolution},
  author={Moriarty, David E and Miikkulainen, Risto},
  journal={Evolutionary Computation},
  volume={5},
  number={4},
  pages={373--399},
  year={1997},
  publisher={MIT Press}
}

@article{saravanan1995evolving,
  title={Evolving neural control systems},
  author={Saravanan, Natarajan and Fogel, David B},
  journal={IEEE Intelligent Systems},
  volume={10},
  number={3},
  pages={23--27},
  year={1995},
  publisher={IEEE Computer Society}
}

@inproceedings{wieland1991evolving,
  title={Evolving neural network controllers for unstable systems},
  author={Wieland, Alexis P},
  booktitle={Neural Networks, 1991., IJCNN-91-Seattle International Joint Conference on},
  volume={2},
  pages={667--673},
  year={1991},
  organization={IEEE}
}


@article{whitley1993genetic,
  title={Genetic Reinforcement Learning for Neurocontrol Problems},
  author={Whitley, Darrell and Dominic, Stephen and Das, Rajarshi and Anderson, Charles W},
  journal={Machine Learning},
  volume={13},
  pages={259--284},
  year={1993}
}

@article{siebel2007evolutionary,
  title={Evolutionary reinforcement learning of artificial neural networks},
  author={Siebel, Nils T and Sommer, Gerald},
  journal={International Journal of Hybrid Intelligent Systems},
  volume={4},
  number={3},
  pages={171--183},
  year={2007},
  publisher={IOS Press}
}

@book{anthony2009neural,
  title={Neural network learning: Theoretical foundations},
  author={Anthony, Martin and Bartlett, Peter L},
  year={2009},
  publisher={cambridge university press}
}


@article{nakata2015xcs,
  title={XCS-SL: a rule-based genetic learning system for sequence labeling},
  author={Nakata, Masaya and Kovacs, Tim and Takadama, Keiki},
  journal={Evolutionary Intelligence},
  pages={1--16},
  year={2015},
  publisher={Springer}
}

@article{kohl2012integrated,
  title={An integrated neuroevolutionary approach to reactive control and high-level strategy},
  author={Kohl, Nate and Miikkulainen, Risto},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={16},
  number={4},
  pages={472--488},
  year={2012},
  publisher={IEEE}
}

@inproceedings{gauci2007generating,
  title={Generating large-scale neural networks through discovering geometric regularities},
  author={Gauci, Jason and Stanley, Kenneth},
  booktitle={Proceedings of the 9th annual conference on Genetic and evolutionary computation},
  pages={997--1004},
  year={2007},
  organization={ACM}
}

@book{koza1992genetic,
  title={Genetic programming: on the programming of computers by means of natural selection},
  author={Koza, John R},
  volume={1},
  year={1992},
  publisher={MIT press}
}

@article{orriols2009fuzzy,
  title={Fuzzy-UCS: a Michigan-style learning fuzzy-classifier system for supervised learning},
  author={Orriols-Puig, Albert and Casillas, Jorge and Bernad{\'o}-Mansilla, Ester},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={13},
  number={2},
  pages={260--283},
  year={2009},
  publisher={IEEE}
}

@article{rosenstein2004supervised,
  title={Supervised Actor-Critic Reinforcement Learning},
  author={Rosenstein, Michael T and Barto, Andrew G and Si, Jennie and Barto, Andy and Powell, Warren and Wunsch, Donald},
  journal={Handbook of Learning and Approximate Dynamic Programming},
  pages={359--380},
  year={2004},
  publisher={Wiley Online Library}
}

@incollection{starzyk2010novel,
  title={A Novel Optimization Algorithm Based on Reinforcement Learning},
  author={Starzyk, Janusz A and Liu, Yinyin and Batog, Sebastian},
  booktitle={Computational Intelligence in Optimization},
  pages={27--47},
  year={2010},
  publisher={Springer}
}

@article{berglund2006parameterless,
  title={The parameterless self-organizing map algorithm},
  author={Berglund, Erik and Sitte, Joaquin},
  journal={Neural Networks, IEEE Transactions on},
  volume={17},
  number={2},
  pages={305--316},
  year={2006},
  publisher={IEEE}
}

@inproceedings{miagkikh1999global,
  title={Global search in combinatorial optimization using reinforcement learning algorithms},
  author={Miagkikh, Victor V and Punch III, William F},
  booktitle={Evolutionary Computation, 1999. CEC 99. Proceedings of the 1999 Congress on},
  volume={1},
  year={1999},
  organization={IEEE}
}

@article{grondman2012survey,
  title={A Survey of Actor-Critic Reinforcement Learning: Standard and Natural Policy Gradients},
  author={Grondman, Ivo and Busoniu, Lucian and Lopes, Gabriel AD and Babuska, Robert},
  journal={Systems, Man, and Cybernetics, Part C: Applications and Reviews, IEEE Transactions on},
  volume={42},
  number={6},
  pages={1291--1307},
  year={2012},
  publisher={IEEE}
}

@article{shao2013swarm,
  title={Swarm robots reinforcement learning convergence accuracy-based learning classifier systems with gradient descent (XCS-GD)},
  author={Shao, Jie and Lin, Haixia and Zhang, Kaibian},
  journal={Neural Computing and Applications},
  pages={1--6},
  year={2013},
  publisher={Springer}
}

@article{kober2013reinforcement,
  title={Reinforcement learning in robotics: A survey},
  author={Kober, Jens and Bagnell, J Andrew and Peters, Jan},
  journal={The International Journal of Robotics Research},
  volume={32},
  number={11},
  pages={1238--1274},
  year={2013},
  publisher={SAGE Publications}
}

@article{van2011insights,
  title={Insights in Reinforcement Learning: formal analysis and empirical evaluation of temporal-difference learning algorithms},
  author={van Hasselt, HP},
  journal={SIKS dissertation series},
  volume={2011},
  number={04},
  year={2011},
  publisher={Utrecht University}
}

@article{barto1983neuronlike,
  title={Neuronlike adaptive elements that can solve difficult learning control problems},
  author={Barto, Andrew G and Sutton, Richard S and Anderson, Charles W},
  journal={Systems, Man and Cybernetics, IEEE Transactions on},
  number={5},
  pages={834--846},
  year={1983},
  publisher={IEEE}
}

@article{rougier2011dynamic,
  title={Dynamic self-organising map},
  author={Rougier, Nicolas and Boniface, Yann},
  journal={Neurocomputing},
  volume={74},
  number={11},
  pages={1840--1847},
  year={2011},
  publisher={Elsevier}
}


@article{yao1997new,
  title={A new evolutionary system for evolving artificial neural networks},
  author={Yao, Xin and Liu, Yong},
  journal={Neural Networks, IEEE Transactions on},
  volume={8},
  number={3},
  pages={694--713},
  year={1997},
  publisher={IEEE}
}

@inproceedings{kassahun2005efficient,
  title={Efficient reinforcement learning through evolutionary acquisition of neural topologies},
  author={Kassahun, Yohannes and Sommer, Gerald},
  booktitle={In 13th European Symposium on Artificial Neural Networks (ESANN)},
  year={2005},
  organization={Citeseer}
}

@article{angeline1994evolutionary,
  title={An evolutionary algorithm that constructs recurrent neural networks},
  author={Angeline, Peter J and Saunders, Gregory M and Pollack, Jordan B},
  journal={Neural Networks, IEEE Transactions on},
  volume={5},
  number={1},
  pages={54--65},
  year={1994},
  publisher={IEEE}
}

@article{haykin2004comprehensive,
  title={A comprehensive foundation},
  author={Haykin, Simon and Network, Neural},
  journal={Neural Networks},
  volume={2},
  number={2004},
  year={2004}
}


@Misc{neatcode,
author = {Stanley, K. and Karpov, I. and Erkin, B. and Thomas, D.},
title = {{NEAT C++}},
howpublished = {\url{http://nn.cs.utexas.edu/keyword?neat-c}},
year = {2001--2011}
}

@article{kohl:nn09,
title={Evolving Neural Networks for Strategic Decision-Making Problems},
author={Nate Kohl and Risto Miikkulainen},
booktitle={Neural Networks, Special issue on Goal-Directed Neural Systems},
url="http://nn.cs.utexas.edu/?kohl:nn09",
year={2009}
}

@inproceedings{kohl2008evolving,
  title={Evolving neural networks for fractured domains},
  author={Kohl, Nate and Miikkulainen, Risto},
  booktitle={Proceedings of the 10th annual conference on Genetic and evolutionary computation},
  pages={1405--1412},
  year={2008},
  organization={ACM}
}

@article{whiteson2006evolutionary,
  title={Evolutionary function approximation for reinforcement learning},
  author={Whiteson, Shimon and Stone, Peter},
  journal={The Journal of Machine Learning Research},
  volume={7},
  pages={877--917},
  year={2006},
  publisher={JMLR. org}
}

@inproceedings{gomez1999solving,
  title={Solving non-Markovian control tasks with neuroevolution},
  author={Gomez, Faustino J and Miikkulainen, Risto},
  booktitle={IJCAI},
  volume={99},
  pages={1356--1361},
  year={1999}
}

@inproceedings{wieland1991evolving,
  title={Evolving neural network controllers for unstable systems},
  author={Wieland, Alexis P},
  booktitle={Neural Networks, 1991., IJCNN-91-Seattle International Joint Conference on},
  volume={2},
  pages={667--673},
  year={1991},
  organization={IEEE}
}

@article{stanley2002evolving,
  title={Evolving neural networks through augmenting topologies},
  author={Stanley, Kenneth and Miikkulainen, Risto},
  journal={Evolutionary computation},
  volume={10},
  number={2},
  pages={99--127},
  year={2002},
  publisher={MIT Press}
}

@article{stanley1996efficient,
  title={Efficient reinforcement learning through evolving neural network topologies},
  author={Stanley, Kenneth O and Miikkulainen, Risto},
  journal={Network (Phenotype)},
  volume={1},
  number={2},
  pages={3},
  year={1996}
}

@inproceedings{sutton1996generalization,
  title={Generalization in Reinforcement Learning: Successful Examples Using Sparse Coarse Coding},
  author={Sutton, Richard S},
  booktitle={Advances in Neural Information Processing Systems 8},
  year={1996}
}

@incollection{bonarini1996evolutionary,
  title={Evolutionary learning of fuzzy rules: competition and cooperation},
  author={Bonarini, Andrea},
  booktitle={Fuzzy Modelling},
  pages={265--283},
  year={1996},
  publisher={Springer}
}

@InProceedings{Twardowski1993a,
  author =       "Kirk Twardowski",
  title =        "{Credit Assignment for Pole Balancing with Learning
                 Classifier Systems}",
  pages =        "238--245",
  crossref =     "ICGA93",
  keywords =     "LCS",
  abstract =     "Effective reinforcement learning methods are essential
                 for credit assignment in learning classifier systems in
                 order to guide the structural rule-base modifications
                 performed by genetic algorithms. Currently, a number of
                 algorithms have been proposed to fulfill this
                 fundamental need; the most frequently employed being
                 the bucket-brigade algorithm. In this paper, an
                 experimental evaluation of a number of reinforcement
                 learning algorithms for a variety of parameter settings
                 is presented. A simplified learning classifier system
                 is used in order to minimize system complexity in order
                 to isolate the behavior of the reinforcement learning
                 algorithms. The problem domain tackled is that of the
                 control of an unstable dynamic system. It was
                 discovered that exploitation of current information is
                 highly favored over exploration for new information and
                 that a hybrid bucket brigade-backward averaging
                 algorithm produced the fastest convergence to a
                 solution.",
}

@inproceedings{vargas2013aself,
  title={Self organizing classifiers and niched fitness},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi},
  booktitle={Proceedings of the fifteenth annual conference on Genetic and evolutionary computation conference},
  pages={1109--1116},
  year={2013},
  organization={ACM}
}

@inproceedings{vargas2015novelty,
  title={Novelty-organizing team of classifiers in noisy and dynamic environments},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi},
  booktitle={Evolutionary Computation, 2015. CEC 2015. IEEE Congress on},
  year={2015},
  organization={IEEE}
}
  pages={1785--1792},

@inproceedings{vargas2014novelty,
  title={Novelty-organizing team of classifiers-A team-individual multi-objective approach to reinforcement learning},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi},
  booktitle={SICE Annual Conference (SICE), 2014 Proceedings of the},
  pages={1785--1792},
  year={2014},
  organization={IEEE}
}

@inproceedings{vargas2013continuous,
  title={Continuous adaptive reinforcement learning with the evolution of Self Organizing Classifiers},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi},
  booktitle={Development and Learning and Epigenetic Robotics (ICDL), 2013 IEEE Third Joint International Conference on},
  pages={1--2},
  year={2013},
  organization={IEEE}
}

@article{vargas2013self,
  title={Self organizing classifiers: first steps in structured evolutionary machine learning},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi},
  journal={Evolutionary Intelligence},
  volume={6},
  number={2},
  pages={57--72},
  year={2013},
  publisher={Springer}
}

@inproceedings{vargas2014noc,
  author    = {Danilo Vasconcellos Vargas and
               Hirotaka Takano and
               Junichi Murata},
  title     = {Novelty-organizing classifiers applied to classification and reinforcement
               learning: towards flexible algorithms},
  booktitle = {Genetic and Evolutionary Computation Conference, {GECCO} '14, Vancouver,
               BC, Canada, July 12-16, 2014, Companion Material Proceedings},
  pages     = {81--82},
  year      = {2014}
}
  crossref  = {DBLP:conf/gecco/2014c},
  url       = {http://doi.acm.org/10.1145/2598394.2598429},
  doi       = {10.1145/2598394.2598429},
  timestamp = {Sat, 12 Jul 2014 16:22:58 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/gecco/VargasTM14},
  bibsource = {dblp computer science bibliography, http://dblp.org}

@inproceedings{knox2010combining,
  title={Combining manual feedback with subsequent MDP reward signals for reinforcement learning},
  author={Knox, W Bradley and Stone, Peter},
  booktitle={Proceedings of the 9th International Conference on Autonomous Agents and Multiagent Systems: volume 1-Volume 1},
  pages={5--12},
  year={2010},
  organization={International Foundation for Autonomous Agents and Multiagent Systems}
}


@article{igel2004no,
  title={{A no-free-lunch theorem for non-uniform distributions of target functions}},
  author={Igel, C. and Toussaint, M.},
  journal={Journal of Mathematical Modelling and Algorithms},
  volume={3},
  number={4},
  pages={313--322},
  issn={1570-1166},
  year={2004},
  publisher={Springer}
}

@article{franco2013gassist,
  title={GAssist vs. BioHEL: critical assessment of two paradigms of genetics-based machine learning},
  author={Franco, Mar{\'\i}a A and Krasnogor, Natalio and Bacardit, Jaume},
  journal={Soft Computing},
  pages={1--29},
  year={2013},
  publisher={Springer}
}

@incollection{bacardit2007data,
  title={Data mining in learning classifier systems: comparing XCS with GAssist},
  author={Bacardit, Jaume and Butz, Martin V},
  booktitle={Learning Classifier Systems},
  pages={282--290},
  year={2007},
  publisher={Springer}
}

@misc{uci2013,
author = "K. Bache and M. Lichman",
year = "2013",
title = "{UCI} Machine Learning Repository",
url = "http://archive.ics.uci.edu/ml",
institution = "University of California, Irvine, School of Information and Computer Sciences" 
} 

@article{unold2005context,
  title={Context-free grammar induction with grammar-based classifier system},
  author={Unold, O},
  journal={Archives of Control Science},
  volume={15},
  number={4},
  pages={681},
  year={2005},
  publisher={POLITECHNIKA SLASKA}
}

@article{dam2008neural,
  title={Neural-based learning classifier systems},
  author={Dam, Hai Huong and Abbass, Hussein A and Lokan, Chris and Yao, Xin},
  journal={Knowledge and Data Engineering, IEEE Transactions on},
  volume={20},
  number={1},
  pages={26--39},
  year={2008},
  publisher={IEEE}
}

@article{wilson2002classifiers,
  title={Classifiers that approximate functions},
  author={Wilson, Stewart W},
  journal={Natural Computing},
  volume={1},
  number={2-3},
  pages={211--234},
  year={2002},
  publisher={Springer}
}

@article{floreano2008neuroevolution,
  title={Neuroevolution: from architectures to learning},
  author={Floreano, Dario and D{\"u}rr, Peter and Mattiussi, Claudio},
  journal={Evolutionary Intelligence},
  volume={1},
  number={1},
  pages={47--62},
  year={2008},
  publisher={Springer}
}

@article{holmes2002learning,
  title={Learning classifier systems: New models, successful applications},
  author={Holmes, John H and Lanzi, Pier Luca and Stolzmann, Wolfgang and Wilson, Stewart W},
  journal={Information Processing Letters},
  volume={82},
  number={1},
  pages={23--30},
  year={2002},
  publisher={Elsevier}
}

@article{holland1977cognitive,
  title={Cognitive systems based on adaptive algorithms},
  author={Holland, John H and Reitman, Judith S},
  journal={ACM SIGART Bulletin},
  number={63},
  pages={49--49},
  year={1977},
  publisher={ACM}
}

@article{booker1989classifier,
  title={Classifier systems and genetic algorithms},
  author={Booker, Lashon B. and Goldberg, David E. and Holland, John H.},
  journal={Artificial intelligence},
  volume={40},
  number={1},
  pages={235--282},
  year={1989},
  publisher={Elsevier}
}

@article{bacardit2009improving,
  title={Improving the scalability of rule-based evolutionary learning},
  author={Bacardit, Jaume and Burke, Edmund K and Krasnogor, Natalio},
  journal={Memetic Computing},
  volume={1},
  number={1},
  pages={55--67},
  year={2009},
  publisher={Springer}
}

@inproceedings{llora2007towards,
  title={Towards better than human capability in diagnosing prostate cancer using infrared spectroscopic imaging},
  author={Llor{\`a}, Xavier and Reddy, Rohith and Matesic, Brian and Bhargava, Rohit},
  booktitle={Proceedings of the 9th annual conference on Genetic and evolutionary computation},
  pages={2098--2105},
  year={2007},
  organization={ACM}
}

@inproceedings{hurst2004self,
  title={A self-adaptive neural learning classifier system with constructivism for mobile robot control},
  author={Hurst, Jacob and Bull, Larry},
  booktitle={Parallel Problem Solving from Nature-PPSN VIII},
  pages={942--951},
  year={2004},
  organization={Springer}
}


@inproceedings{butz2008context,
  title={Context-dependent predictions and cognitive arm control with XCSF},
  author={Butz, Martin V and Herbort, Oliver},
  booktitle={Proceedings of the 10th annual conference on Genetic and evolutionary computation},
  pages={1357--1364},
  year={2008},
  organization={ACM}
}


@inproceedings{van2009using,
  title={Using continuous action spaces to solve discrete problems},
  author={van Hasselt, Hado and Wiering, Marco A},
  booktitle={Neural Networks, 2009. IJCNN 2009. International Joint Conference on},
  pages={1149--1156},
  year={2009},
  organization={IEEE}
}

@inproceedings{lanzi2006classifier,
  title={Classifier prediction based on tile coding},
  author={Lanzi, Pier Luca and Loiacono, Daniele and Wilson, Stewart W and Goldberg, David E},
  booktitle={Proceedings of the 8th annual conference on Genetic and evolutionary computation},
  pages={1497--1504},
  year={2006},
  organization={ACM}
}

@article{whiteson2006evolutionary,
  title={Evolutionary function approximation for reinforcement learning},
  author={Whiteson, Shimon and Stone, Peter},
  journal={The Journal of Machine Learning Research},
  volume={7},
  pages={877--917},
  year={2006},
  publisher={JMLR. org}
}

@article{fritzke1995growing,
  title={A growing neural gas network learns topologies},
  author={Fritzke, Bernd and others},
  journal={Advances in neural information processing systems},
  volume={7},
  pages={625--632},
  year={1995},
  publisher={MORGAN KAUFMANN PUBLISHERS}
}

@book{kohonen2001self,
  title={Self-organizing maps},
  author={Kohonen, Teuvo},
  volume={30},
  year={2001},
  publisher={Springer}
}

@inproceedings{wiering2011reinforcement,
  title={Reinforcement learning algorithms for solving classification problems},
  author={Wiering, Marco A and van Hasselt, Hado and Pietersma, A-D and Schomaker, Lambert},
  booktitle={Adaptive Dynamic Programming And Reinforcement Learning (ADPRL), 2011 IEEE Symposium on},
  pages={91--96},
  year={2011},
  organization={IEEE}
}

@article{to_appear,
  title={General Subpopulation Framework and Taming the Conflict Inside Populations},
  author={Vargas, Danilo Vasconcellos and Takano, Hirotaka and Murata, Junichi and Delbem, Alexandre Cl\'{a}udio Botazzo},
  journal={Evolutionary computation},
  note={In press},
  publisher={MIT Press}
}

@article{lehman2011abandoning,
  title={Abandoning objectives: Evolution through the search for novelty alone},
  author={Lehman, Joel and Stanley, Kenneth O},
  journal={Evolutionary computation},
  volume={19},
  number={2},
  pages={189--223},
  year={2011},
  publisher={MIT Press}
}

@inproceedings{reehuis2013novelty,
  title={Novelty and interestingness measures for design-space exploration},
  author={Reehuis, Edgar and Olhofer, Markus and Emmerich, Michael and Sendhoff, Bernhard and B{\"a}ck, Thomas},
  booktitle={Proceeding of the fifteenth annual conference on Genetic and evolutionary computation conference},
  pages={1541--1548},
  year={2013},
  organization={ACM}
}

@incollection{iqbal2012xcsr,
  title={XCSR with computed continuous action},
  author={Iqbal, Muhammad and Browne, Will N and Zhang, Mengjie},
  booktitle={AI 2012: Advances in Artificial Intelligence},
  pages={350--361},
  year={2012},
  publisher={Springer}
}

@article{lanzi2007generalization,
  title={Generalization in the {XCSF} classifier system: Analysis, improvement, and extension},
  author={Lanzi, P.L. and Loiacono, D. and Wilson, S.W. and Goldberg, D.E.},
  journal={Evolutionary Computation},
  volume={15},
  number={2},
  pages={133--168},
  year={2007},
  publisher={MIT Press}
}

@inproceedings{lanzi1997study,
  title={A Study of the Generalization Capabilities of {XCS}},
  author={Lanzi, P.L. and others},
  booktitle={Proceedings of the Seventh International Conference on Genetic Algorithm},
  pages={418--425},
  year={1997}
}

@inproceedings{Hutchinson1957,
  title={Concluding Remarks},
  author={Hutchinson, G.E.},
  booktitle={Cold Spring Harbor Symposia on Quantitative Biology 22},
  pages={415--427},
  year={1957}
}

@conference{vesterstrom2004comparative,
  title={{A comparative study of differential evolution, particle swarm optimization, and evolutionary algorithms on numerical benchmark problems}},
  author={Vesterstrom, J. and Thomsen, R.},
  booktitle={Evolutionary Computation, 2004. CEC2004. Congress on},
  volume={2},
  pages={1980--1987},
  isbn={0780385152},
  year={2004},
  organization={IEEE}
}

@article{butz2008function,
  title={Function approximation with {XCS}: Hyperellipsoidal conditions, recursive least squares, and compaction},
  author={Butz, M.V. and Lanzi, P.L. and Wilson, S.W.},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={12},
  number={3},
  pages={355--376},
  year={2008},
  publisher={IEEE}
}



@article{iorio2005solving,
  title={Solving rotated multi-objective optimization problems using differential evolution},
  author={Iorio, A. and Li, X.},
  journal={AI 2004: Advances in Artificial Intelligence},
  pages={861--872},
  year={2005},
  publisher={Springer}
}

@article{garcia2009study,
  title={{A study on the use of non-parametric tests for analyzing the evolutionary algorithms' behaviour: a case study on the CEC'2005 special session on real parameter optimization}},
  author={Garc{\'\i}a, S. and Molina, D. and Lozano, M. and Herrera, F.},
  journal={Journal of Heuristics},
  volume={15},
  number={6},
  pages={617--644},
  issn={1381-1231},
  year={2009},
  publisher={Springer}
}

@inproceedings{goldberg1987genetic,
  title={Genetic algorithms with sharing for multimodal function optimization},
  author={Goldberg, David E and Richardson, Jon},
  booktitle={Genetic algorithms and their applications: Proceedings of the Second International Conference on Genetic Algorithms},
  pages={41--49},
  year={1987},
  organization={Hillsdale, NJ: Lawrence Erlbaum}
}


@article{storn1997differential,
  title={{Differential evolution--a simple and efficient heuristic for global optimization over continuous spaces}},
  author={Storn, R. and Price, K.},
  journal={Journal of global optimization},
  volume={11},
  number={4},
  pages={341--359},
  issn={0925-5001},
  year={1997},
  publisher={Springer}
}

@article{brest2006self,
  title={Self-adapting control parameters in differential evolution: A comparative study on numerical benchmark problems},
  author={Brest, J. and Greiner, S. and Boskovic, B. and Mernik, M. and Zumer, V.},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={10},
  number={6},
  pages={646--657},
  issn={1089-778X},
  year={2006},
  publisher={IEEE}
}

@inproceedings{belding1995distributed,
  title={The Distributed Genetic Algorithm Revisited},
  author={Belding, T.C.},
  booktitle={Proceedings of the Sixth International Conference on Genetic Algorithms: University of Pittsburgh, July 15-19, 1995},
  pages={114},
  year={1995},
  organization={Morgan Kaufmann Pub}
}

@INPROCEEDINGS{manderick1989,
AUTHOR = "Bernard Manderick and Piet Spiessens",
TITLE = "Fine-Grained Parallel Genetic Algorithms.",
booktitle = "ICGA'89",
PAGES = {428-433},
YEAR = {1989}  }

@inproceedings{howard2009towards,
  title={Towards continuous actions in continuous space and time using self-adaptive constructivism in neural {XCSF}},
  author={Howard, G.D. and Bull, L. and Lanzi, P.L.},
  booktitle={Proceedings of the 11th Annual conference on Genetic and evolutionary computation},
  pages={1219--1226},
  year={2009},
  organization={ACM}
}

@article{bonarini2000fuzzy,
  title={Fuzzy and crisp representations of real-valued input for learning classifier systems},
  author={Bonarini, A. and Bonacina, C. and Matteucci, M.},
  journal={Learning Classifier Systems},
  pages={107--124},
  year={2000},
  publisher={Springer}
}



@inproceedings{butz2008context,
  title={Context-dependent predictions and cognitive arm control with {XCSF}},
  author={Butz, M.V. and Herbort, O.},
  booktitle={Proceedings of the 10th annual conference on Genetic and evolutionary computation},
  pages={1357--1364},
  year={2008},
  organization={ACM}
}

@article{stalph2012learning,
  title={Learning local linear Jacobians for flexible and adaptive robot arm control},
  author={Stalph, P.O. and Butz, M.V.},
  journal={Genetic programming and evolvable machines},
  volume={13},
  number={2},
  pages={137--157},
  year={2012},
  publisher={Springer}
}

@inproceedings{tran2007xcsf,
  title={{XCSF} with computed continuous action},
  author={Tran, H.T. and Sanza, C. and Duthen, Y. and Nguyen, T.D.},
  booktitle={Genetic And Evolutionary Computation Conference: Proceedings of the 9 th annual conference on Genetic and evolutionary computation},
  volume={7},
  number={11},
  pages={1861--1869},
  year={2007}
}

@article{bull2002using,
  title={On using constructivism in neural classifier systems},
  author={Bull, L.},
  journal={Parallel problem solving from nature-PPSN VII},
  pages={558--567},
  year={2002},
  publisher={Springer}
}

@article{casillas2007fuzzy,
  title={{Fuzzy-XCS}: A Michigan genetic fuzzy system},
  author={Casillas, J. and Carse, B. and Bull, L.},
  journal={Fuzzy Systems, IEEE Transactions on},
  volume={15},
  number={4},
  pages={536--550},
  year={2007},
  publisher={IEEE}
}

@inproceedings{bull2002accuracy,
  title={Accuracy-based neuro and neuro-fuzzy classifier systems},
  author={Bull, L. and O'Hara, T.},
  booktitle={Proceedings of the Genetic and Evolutionary Computation Conference},
  pages={905--911},
  year={2002},
  organization={Morgan Kaufmann Publishers Inc.}
}

@inproceedings{lanzi2005xcs,
  title={{XCS} with computed prediction in multistep environments},
  author={Lanzi, P.L. and Loiacono, D. and Wilson, S.W. and Goldberg, D.E.},
  booktitle={Proceedings of the 2005 conference on Genetic and evolutionary computation},
  pages={1859--1866},
  year={2005},
  organization={ACM}
}

@inproceedings{valenzuela1991fuzzy,
  title={The fuzzy classifier system: A classifier system for continuously varying variables},
  author={Valenzuela-Rend{\'o}n, M.},
  booktitle={Proceedings of the Fourth International Conference on Genetic Algorithms pp346-353, Morgan Kaufmann I},
  volume={991},
  pages={223--230},
  year={1991}
}

@inproceedings{Widrow1960Adaptive,
    address = {New York},
    author = {Widrow, Bernard and Hoff, Marcian E.},
    booktitle = {1960 {IRE} {WESCON} Convention Record, Part 4},
    citeulike-article-id = {2510415},
    citeulike-linkout-0 = {http://isl-www.stanford.edu/\~{}widrow/papers/c1960adaptiveswitching.pdf},
    keywords = {neural-networks},
    pages = {96--104},
    posted-at = {2010-06-11 17:12:34},
    priority = {2},
    publisher = {{IRE}},
    title = {{Adaptive Switching Circuits}},
    url = {http://isl-www.stanford.edu/\~{}widrow/papers/c1960adaptiveswitching.pdf},
    year = {1960}
}

@article{mouret2011novelty,
  title={Novelty-based multiobjectivization},
  author={Mouret, J.B.},
  journal={New Horizons in Evolutionary Robotics},
  pages={139--154},
  year={2011},
  publisher={Springer}
}

@article{horn1994implicit,
  title={Implicit niching in a learning classifier system: Nature's way},
  author={Horn, J. and Goldberg, D.E. and Deb, K.},
  journal={Evolutionary Computation},
  volume={2},
  number={1},
  pages={37--66},
  year={1994},
  publisher={MIT Press}
}

@inproceedings{alba2000cellular,
  title={Cellular evolutionary algorithms: Evaluating the influence of ratio},
  author={Alba, E. and Troya, J.},
  booktitle={Parallel Problem Solving from Nature PPSN VI},
  pages={29--38},
  year={2000},
  organization={Springer}
}

@article{alba2002parallelism,
  title={Parallelism and evolutionary algorithms},
  author={Alba, E. and Tomassini, M.},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={6},
  number={5},
  pages={443--462},
  year={2002},
  publisher={IEEE}
}

@book{tomassini2005spatially,
  title={Spatially structured evolutionary algorithms},
  author={Tomassini, M.},
  year={2005},
  publisher={Springer}
}

@article{butz2004toward,
  title={Toward a theory of generalization and learning in {XCS}},
  author={Butz, M.V. and Kovacs, T. and Lanzi, P.L. and Wilson, S.W.},
  journal={Evolutionary Computation, IEEE Transactions on},
  volume={8},
  number={1},
  pages={28--46},
  year={2004},
  publisher={IEEE}
}

@article{butz2001algorithmic,
  title={An algorithmic description of {XCS}},
  author={Butz, M. and Wilson, S.},
  journal={Advances in Learning Classifier Systems},
  pages={267--274},
  year={2001},
  publisher={Springer}
}

@article{butz2001algorithmic,
  title={An algorithmic description of {XCS}},
  author={Butz, M. and Wilson, S.},
  journal={Advances in Learning Classifier Systems},
  pages={267--274},
  year={2001},
  publisher={Springer}
}

@article{wilson2002classifiers,
 author = {Wilson, Stewart W.},
 title = {Classifiers that approximate functions},
 issue_date = {June 2002},
 volume = {1},
 number = {2-3},
 month = jun,
 year = {2002},
 issn = {1567-7818},
 pages = {211--234},
 numpages = {24},
 url = {http://dx.doi.org/10.1023/A:1016535925043},
 doi = {10.1023/A:1016535925043},
 acmid = {599708},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
 keywords = {classifier systems, continuous actions, function approximation, generalized classifier},
} 

@article{kohonen1998self,
  title={The self-organizing map},
  author={Kohonen, T.},
  journal={Neurocomputing},
  volume={21},
  number={1},
  pages={1--6},
  year={1998},
  publisher={Elsevier}
}

@article{kohonen1990self,
  title={The self-organizing map},
  author={Kohonen, T.},
  journal={Proceedings of the IEEE},
  volume={78},
  number={9},
  pages={1464--1480},
  year={1990},
  publisher={IEEE}
}

@phdthesis{Booker:1982:IBA:910371,
 author = {Booker, Lashon Bernard},
 title = {Intelligent behavior as an adaptation to the task environment},
 year = {1982},
 note = {AAI8214966},
 publisher = {University of Michigan},
 address = {Ann Arbor, MI, USA},
} 

@article{wilson1995classifier,
  title={Classifier fitness based on accuracy},
  author={Wilson, S.W.},
  journal={Evolutionary computation},
  volume={3},
  number={2},
  pages={149--175},
  year={1995},
  publisher={MIT Press}
}

@article{lanzi2000roadmap,
  title={A roadmap to the last decade of learning classifier system research (from 1989 to 1999)},
  author={Lanzi, P. and Riolo, R.},
  journal={Learning Classifier Systems},
  pages={33--61},
  year={2000},
  publisher={Springer}
}

@article{urbanowicz2009learning,
  title={Learning classifier systems: a complete introduction, review, and roadmap},
  author={Urbanowicz, R.J. and Moore, J.H.},
  journal={Journal of Artificial Evolution and Applications},
  volume={2009},
  pages={1},
  year={2009},
  publisher={Hindawi Publishing Corp.}
}

@article{bacardit2006biohel,
  title={Biohel: Bioinformatics-oriented hierarchical evolutionary learning},
  author={Bacardit, J. and Krasnogor, N.},
  year={2006},
  publisher={Computer Science \& IT}
}

@inproceedings{llora2007towards,
  title={Towards better than human capability in diagnosing prostate cancer using infrared spectroscopic imaging},
  author={Llor{\`a}, X. and Reddy, R. and Matesic, B. and Bhargava, R.},
  booktitle={Proceedings of the 9th annual conference on Genetic and evolutionary computation},
  pages={2098--2105},
  year={2007},
  organization={ACM}
}

@ARTICLE{wilson1994zcs,
  TITLE= "{ZCS}: A zeroth level classifier system",
  author={Wilson, S.W.},
  journal={Evolutionary computation},
  volume={2},
  number={1},
  pages={1--18},
  year={1994},
  publisher={MIT Press}
}



@ARTICLE{bowman:reasoning,
	AUTHOR = "Mic Bowman and Saumya K. Debray and Larry L. Peterson",
	TITLE = "Reasoning About Naming Systems",
	JOURNAL = "ACM Trans. Program. Lang. Syst.",
	VOLUME = {15},
	NUMBER = {5},
	PAGES = {795-825},
	MONTH = "November",
	YEAR = {1993}	}

@ARTICLE{braams:babel,
	AUTHOR = "Johannes Braams",
	TITLE = "Babel, a Multilingual Style-Option System for Use with LaTeX's Standard Document Styles",
	JOURNAL = {TUGboat},
	VOLUME = {12},
	NUMBER = {2},
	PAGES = {291-301},
	MONTH = "June",
	YEAR = {1991}	}

@INPROCEEDINGS{clark:pct,
	AUTHOR = "Malcolm Clark",
	TITLE = "Post Congress Tristesse",
	BOOKTITLE = "TeX90 Conference Proceedings",
	PAGES = "84-89",
	ORGANIZATION = "TeX Users Group",
	MONTH = "March", 
	YEAR = {1991}	}

@ARTICLE{herlihy:methodology,
	AUTHOR = "Maurice Herlihy",
	TITLE = "A Methodology for Implementing Highly Concurrent
	Data Objects",
	JOURNAL = {ACM Trans. Program. Lang. Syst.},
	VOLUME = {15},
	NUMBER = {5},
	PAGES = {745-770},
	MONTH = "November",
	YEAR = {1993}	}

@BOOK{Lamport:LaTeX,
	AUTHOR = "Leslie Lamport",
	TITLE = "LaTeX User's Guide and Document Reference Manual",
	PUBLISHER = "Addison-Wesley Publishing Company",
	ADDRESS = "Reading, Massachusetts",
	YEAR = "1986"	}

@BOOK{salas:calculus,
	AUTHOR = "S.L. Salas and Einar Hille",
	TITLE = "Calculus: One and Several Variable",
	PUBLISHER = "John Wiley and Sons",
	ADDRESS = "New York",
	YEAR = "1978"	}







